Rigorous validation of a Hopf bifurcation in the Kuramoto-Sivashinsky PDE

We use computer-assisted proof techniques to prove that a branch of non-trivial equilibrium solutions in the Kuramoto-Sivashinsky partial differential equation undergoes a Hopf bifurcation. Furthermore, we obtain an essentially constructive proof of the family of time-periodic solutions near the Hopf bifurcation. To this end, near the Hopf point we rewrite the time periodic problem for the Kuramoto-Sivashinsky equation in a desingularized formulation. We then apply a parametrized Newton-Kantorovich approach to validate a solution branch of time-periodic orbits. By construction, this solution branch includes the Hopf bifurcation point.

==> abstract_PDE.tex <==
%<*abstract-PDE>

%It is usually very difficult to prove analytically  the existence of bifurcations in partial differential equations. 

We use computer-assisted proof techniques to prove that a branch of  non-trivial equilibrium solutions in the Kuramoto–Sivashinsky partial differential equation undergoes a Hopf bifurcation. 
Furthermore, we obtain an essentially constructive proof of the family of
time-periodic solutions near the Hopf bifurcation. To this end, near the Hopf point we rewrite the time periodic problem for the Kuramoto–Sivashinsky equation in a desingularized formulation. 
We then apply a parametrized Newton-Kantorovich approach to validate a solution branch of time-periodic orbits. By contruction, this solution branch includes the Hopf bifurcation point. 

%</abstract-PDE>

==> bounds-single.tex <==
%<*bounds-single>

For ease of exposition, in this section we  present the explicit computation of the bounds  introduced in Equations \eqref{general_Y} and \eqref{generalZ} for the case of a single solution. In Section~\ref{s:boundsparametrization} we generalize this to validated continuation of solution branches.The approximate numerical solution considered is denoted by $\hat x=(\hat \lambda, \hat v)$, and the zero finding problem is  of the form $H(x)=(G(x),F(x))=0$,  with $F$ and $G$ defined in~\eqref{F} and~\eqref{e:defG}, respectively, are now $s$-\emph{independent}.

\subsection{Constructing the Newton-like operator $T$}
\label{s:constructA}

 
In order to apply the radial polynomial approach to validate a numerical solution $\hat x$, we construct a Newton-like operation $T$ by using $A$, the approximate inverse of $DH(\emb \hat x)$. The first step is the construction of $A^\dagger$, a  (partly numerical) approximation of $DH(\emb \hat x)$, on which we will base our construction of $A$.

We split  $A$ and $A^\dagger$ into a finite part, defined numerically and stored in the computer, and an infinite part, called the tail, defined analytically. The finite part of $A^\dagger$ is chosen to be the finite dimensional Jacobian $D\hat{H}(\hat{x})$. The finite part of $A$ is an numerically computed \emph{approximate} inverse $\hat{A}$ of $D\hat{H}(\hat{x})$, where~$\hat{H}$ is defined in~\eqref{e:defhatH}. For the tail of $A^\dagger$ the dominant term $\imag  k (v_n)_k$ is the natural candidate, while for the tail of $A$  the corresponding  choice is thus $\imag k^{-1}(v_n)_k$.
 
%** use notation of finite Jacobian
To be precise, we define $A$ and  $A^\dagger$ through
\begin{align}
\qquad & A^\dagger x \bydef
\emb \left(D\hat{H}(\hat{x})\,\Pi_Kx\right)-\imag \boldsymbol{K} \IK x ,
\label{operator_Adagger}
\\
\qquad & A x \bydef
\emb \left(\hat{A}\,\Pi_K x\right)-\imag \boldsymbol{K}^{-1} \IK x, 
\label{operator_A}
\end{align}
where %$\hat{A}$ is defined as a finite numerical approximation of the inverse of $D\hat{H}(\hat{x})$ and 
$$
(\boldsymbol{K}x)_n \bydef \begin{cases}
0 &\text{for } n = 1,\dots,M\\
\boldsymbol{k}x_n & \text{for } n = M+1,\dots, M+N,
\end{cases}
$$
and
$$
(\boldsymbol{K}^{-1}x)_n \bydef \begin{cases}
0 &\text{for } n = 1,\dots,M\\
\boldsymbol{k}^{-1}x_n &\text{for } n = M+1,\dots, M+N,
\end{cases}
$$
with (see also~\eqref{e:boldk})
\begin{equation*}
	(\boldsymbol{k} w)_k \bydef k w_k \qquad \text{and}\qquad
	(\boldsymbol{k}^{-1} w)_k \bydef
	\begin{cases}
		0 & \text{if }k=0 \\
		k^{-1} w_k & \text{if } k\in \Z\setminus\{0\}.
	\end{cases}
\end{equation*} 

\begin{remark}\label{r:IAAnotail}
The tails of $A$ and $A^\dagger$ are exact inverses, hence
\begin{equation}\label{e:IAA}
  I - A A^\dagger = \embPi_K - \emb (\hat{A} \, D\hat{H}(\hat{x})) \Pi_K ,
\end{equation}
i.e., $I - A A^\dagger$ is represented by a matrix.
\end{remark}
\begin{remark}\label{sizeAx}
Since the tail of $A$ is diagonal, when $x$ has at most $K'$ nonzero modes, then $Ax$ has at most $\max\{K,K'\}$ nonzero modes.
% When $A$, defined in \eqref{operator_A} depending on $K$, is applied to a vector $x$ that has at most $k$ non-zero modes, i.e., such that $\emb\Pi_k x =x$, then $Ax$ has at most $\tilde{k} = \max(K,k)$ non-zero modes:
% $$
% \emb \Pi_{\tilde{k}} A x = A x,
% $$
% since the diagonal tail $\boldsymbol{K}^{-1} I_K$, determined by $K$, preserves the zero nodes.
%with $\tilde{k} = \max ( K, k)$.
\end{remark}

% We emphasize that $A$ is the combination of a numerical finite part $\hat A$
% and an analytical tail, and we can therefore compute all the elements of
% $\Pi_kA\Pi_k$ at any time up to any finite $k$ once the numerical finite part
% is stored.
We note that $A$ has the structure assumed in Lemma~\ref{lem:weird_matrix}. Moreover, even though $H$ does not map $\XX$ into itself, we observe that $AH(x) \in\XX \qquad \text{for all } x \in \XX$. In particular,
%Now that we have defined the action of $A$, we set
\begin{align*}
T:
%\,\XX&\rightarrow \XX\\ban
x&\mapsto x-AH(x)
\end{align*}
maps  $\XX$ to itself, cf.~Proposition 4 in \cite{hungria-lessard}.


Having defined the fixed point operator $T$, we now derive explicit bounds $Y$ and $Z$ satisfying~\eqref{general_Y} and~\eqref{general_Z} in Sections~\ref{s:singleY} and~\ref{s:singleZ}, respectively.



\subsection{The $Y$ bound}
\label{s:singleY}

In this section, we are interested in computing the $Y$ bound, that is the $M+N$ vector such that
\begin{equation}\label{Yloc}
Y_n \geq \left\| [T(\emb\hat{x}) - \emb\hat{x}]_n\right\|=\left\| [AH(\emb\hat{x})]_n\right\|, \qquad \text{for }n=1,\dots,M+N. 
\end{equation}
%where $AH(\emb\hat{x})$ is an  element in $\XX$. 
Since $\hat{x}$ has $K$ non-zero modes, by Remark \ref{finite_conv} we know that $H(\emb\hat{x})$ will have at most  $K|D|$ non-zero modes (we recall that $|D|$ is the order of the polynomial vector field). Remark~\ref{sizeAx} implies that $AH(\emb\hat{x})$ has at most $K|D|$ non-zero modes, all of which can be computed explicitly in a finite number of operations. By performing these operations with interval arithmetic we obtain bounds satisfying \eqref{Yloc}.
%a finite number of non-zero elements, bounded by the indices $-K|D|$ and $K|D|$.
%\red{$|D|$ hasn't been defined yet.}


%Since $\hat{x}$ is a finite vector, by construction  also $H(\emb\hat{x})$ is finite. In particular since the vector field is polynomial, for $i=M+1,\dots ,M+N$,  $[H(\emb\hat{x})]_i$  has at most $|D|(2K+1)$  non-zero elements, as stated in  Remark \ref{finite_conv}, therefore the computations can be done explicitly using Equation \eqref{operator_norm}.


\subsection{The splitting of the $Z$ bound}
\label{s:singleZ}

In view of  \eqref{generalZ}, the $Z$ bound for the non-continuation case needs to satisfy
\begin{equation}\label{general_Z}
Z_n(r) \geq \sup_{b,c\in B_r(0)}\|[  DT(\emb\hat{x}+b)c]_n\|,\qquad \text{for }n=1,\dots, M+N.
\end{equation}
% that differs from the general case since in this case the maximization over $s$ is not needed.
We split the estimate into three parts:
% The norm can be split into three parts %and we take care of each part separately, that is
\begin{align}\label{e:splitZ}
\sup_{b,c\in B_r(0)}\| [DT(\emb\hat{x}+&b)c]_n\| \leq \underbrace{ \sup_{c\in B_r(0)} \| [(I - AA^\dagger)c]_n\|}_{\leq Z_{0n}r} \\
& \mbox{} +\underbrace{\sup_{c\in B_r(0)} \|[A( DH(\emb\hat{x})-A^\dagger )c]_n\|}_{ \leq Z_{1n}r} \nonumber\\
&\mbox{} +\underbrace{ \sup_{b,c\in B_r(0)} \|[A(DH(\emb\hat{x}) - DH(\emb\hat{x}+b))c ]_n\|}_{\leq \tilde{Z}_{2n}(r)},
\end{align}
where the first two parts are linear in $r$. We deal with the $Z_{0n}$, $Z_{1n}$ and $Z_{2n}$ bounds separately.
%In the standard case, often the terms here labeled ad $Z_2$ and $Z_1$ are not split, 

%In other approaches, such as \cite{castelli} and \cite{hungria-lessard}, the terms here labeled as $Z_2$ and $Z_1$ are computed together as a polynomial of order $|D|$ in $r$,
%therefore leading to more precise bounds, but the draw back is that it would require more knowledge of the vector field in order to compute the radii polynomials up to order $|D|$. In this presentation, we prefer to simplify the approach and have a rougher bound.
%This splitting is useful because it allows to have two finite-dimensional computations, as we will prove for $Z_0$ and $Z_1$. The last computation will be paired with a second power of $r$, therefore allowing us to have a rough estimate but still good radii polynomials. 

\subsubsection{The $Z_0$ bound}
\label{Z0bound}

Rescaling $c \to cr$, the $Z_0$ bounds have been defined as satisfying
$$
Z_{0n} \geq\sup_{c\in B_1(0)}\| [(I-AA^\dagger)c]_n\|.\label{e:Z0n}
$$
By using~\eqref{e:IAA} we obtain
%and using the previous definitions, we have
\begin{align}
\| [(I-AA^\dagger)c]_n\| &\leq \| [(I-AA^\dagger)\embPi_Kc] + [(I-AA^\dagger)\IK c]_n\|  \nonumber \\
% &= \| [(\Pi_K I - \hat{A} D\hat{H}(\hat{x}))\Pi_K c]_n + [I_K(I- K^{-1}K) I_K 
% c]_n\| \\
% &= \| [(\Pi_K I - \hat{A} D\hat{H}(\hat{x}))\Pi_K c]_n + [I_KI_(I- I) I_K 
% c]_n\| \\
&= \|  (\embPi_K - \emb  \hat{A} D\hat{H}(\hat{x})\Pi_K) c]_n \|.  \nonumber
\end{align}
Here $\embPi_K - \emb  \hat{A} D\hat{H}(\hat{x})\Pi_K $  can be represented as a finite matrix, hence we compute explicit bounds~\eqref{e:Z0n} by applying Lemma~\ref{operator_norm_lemma} and using~\eqref{fin_op_norm}.

\subsubsection{The $Z_1$ bound}
\label{Z1bound}

%\nope
Rescaling $c \to cr$, we aim to find bounds of the form
\begin{equation}\label{e:Z1n}
Z_{1n} \geq\sup_{c\in B_1(0)} \|[A(A^\dagger-DH(\emb\hat{x}))c]_n\|.
\end{equation}
We first analyse the operator
\[
  B = A^\dagger-DH(\emb\hat{x}).
\]
It follows form the definition~\eqref{operator_Adagger} of $A^\dagger$ that $B_{nm}=0$ for $n=1,\dots,M$ and $m=1,\dots,M+N$. Furthermore, for $n=M+1,\dots,M+N$ and $m=1,\dots n$, we have that $B_{nm}$ has at most $K |D|$ nonzero modes, and $\Pi_K B_{nm} =0$. Finally, it follows from~\eqref{e:DmFn} that
\[
  B_{nm} =  \toep_{\hf^{e_{m}}_{n-M}(\emb\hat{x})} 
  						- \embtPi_K \toep_{\hf^{e_{m}}_{n-M}(\emb\hat{x})} \embtPi_K 
  \qquad\text{for } n,m =M+1,\dots, M+N,
\]
which has bandwidth at most $K(|D|-1)$.

\begin{remark}\label{r:product}
Before we proceed, consider the product $Q_1 Q_2$ of two operators in $B(\ell^1_\nu,\ell^1_\nu)$ of the form
\begin{alignat*}{1}
  Q_1 &= \embt \hat{Q}_1 \tPi_K + \imag \boldsymbol{k}^{-1} (I-\tPi_K) , \\
  Q_2 &= \embt \hat{Q}_2 \tPi_K + \toep_{y},
\end{alignat*}
for some $(2K+1) \times (2K+1)$ matrices $\hat{Q}_1$ and $\hat{Q}_2$, and an element $y \in \ell^1_\nu$ with at most $K'$ nonzero modes. Then the product $Q = Q_1 Q_2$ is of the form described in Lemma~\ref{lem:weird_matrix} with $K_1=K+2K'$, $K_2=K+K'$ and $y^*=\frac{1}{K+1} y$, i.e.~$K_3=K'$.
\end{remark}

%\red{This needs to be checked for correctness.}
For the product operator $AB=A(A^\dagger-DH(\emb\hat{x}))$  we find that $(AB)_{nm}=0$ for $n,m=1,\dots,M$. Furthermore, $(AB)_{nm}$ has at most $K|D|$ nonzero modes for $n=1,\dots,M$ and $m=M+1,\dots,M+N$, as well as for $n=M+1,\dots,M+N$ and $m=1,\dots,M$.  Finally, for $n,m=M+1,\dots,M+N$, based on Remark~\ref{r:product} we conclude that $(AB)_{nm}$ is of the form described in Lemma~\ref{lem:weird_matrix}, with $K_1=K|D|$, $K_2=K(2|D|-1)$ and $K_3=K(|D|-1)$ and $y_*= \frac{1}{K+1}  |\hf^{e_{m}}_{n-M}(\hat{x})|$. 
%\red{Elena: is this the size used in the code? yes}

We thus determine the bounds~\eqref{e:Z1n} explicitly by a direct computation based on Lemmas~\ref{operator_norm_lemma} and~\ref{lem:weird_matrix}. 



%Let us consider again 
%\begin{align*}
%\left\|\left(A[A^\dagger-D{H}(\hat{x})]c\right)_i\right\|_\nu&= \left\|\sum_{j=1}^{M+N}\left( A\left[ A^\dagger-D{H}(\hat{x})\right]\right)_{ij}\bar{c}_j\right\|_\nu r\\
%&\leq \sum_{j=1}^{M+N} \left\|  \sum_{l=1}^{M+N} A_{is}\left[ A^\dagger -D{H}(\hat{x})\right]_{lj} \bar{c}_j \right\|_\nu
%\end{align*}
%where
%\begin{align*}
%D{H}(\hat{x}) _{lj}= \begin{cases}
%D_j{G}_s(\hat{x})=A^\dagger_{lj} \quad &l=1,\dots,M,\\
%D_j{F}_l(\hat{x}) \quad &l=M+1,\dots,M+N,
%\end{cases}
%\end{align*}
%and it is reminded that
%\begin{align*}
%&\sum_j D_j{F}_l(\hat{x})y_j=\sum_{d\in D} (f_d)_l d_j x^{d-e_j}y_j -\mathbf{i} \tilde{b}_l -\mathbf{i} \tilde{a}_s,\\
%&\sum_jA^\dagger_{lj}y_j=\sum_{d\in D} (f_d)_l d_j \left(\left(x^{d-e_j}\right)^{(F)}y_j^{(F)} \right)^{(F)} - \mathbf{i}\tilde{b}_l^{(F)} -\mathbf{i}\tilde{a}_l^{(F)},\\
%&\sum_jA_{il}\left( D_j{F}_l(\hat{x})-A^\dagger_{lj}\right)c_j = \sum_j A_{il}\sum_{d\in D}(f_d)_ld_j\left[   
%x^{d-e_j}y_j-\left(  (x^{d-e_j})^{(F)} y_j^{(F)}\right)^{(F)}
%\right] - A_{il} \mathbf{i}  \tilde{b}_l^{(I)}.
%\end{align*}
%At this point, assuming $\| y\|\leq 1$, the terms fall into three categories, i.e.:
%\begin{itemize}
%\item  the terms of the form $A_{il}\mathbf{i}\tilde{b}_s^{(I)}$, that can be bounded by $\tilde{K}_{is}$;
%\item  the terms in the form $A_{il}(f_d)_l d_j\left[   
%x^{d-e_j}y_j-\left(  (x^{d-e_j})^{(F)} y_j^{(F)}\right)^{(F)}
%\right]$, when $d-e_j$ is different than zero, that can be bounded by $\frac{|(f_d)_s|\|x^{d-e_j}\|_\nu}{(m+1)}+\sum_{|n|\leq N}\sum_{|k|\leq N} \left | \left(A_{il}\right)_{n,k}\right| \Psi_k(x^{d-e_j})$;
%\item  the terms in the form $A_{il}(f_d)_sd_j\left[   
%x^{d-e_j}y_j-\left(  (x^{d-e_j})^{(F)} y_j^{(F)}\right)^{(F)}
%\right]$, when $d-e_j$ is zero, than can be bounded by $\frac{|(f_d)_s|}{(m+1)}$.
%\end{itemize}
%
%Let us first remark that $D_jH_l(\hat{x})$ can be viewed as an infinite matrix applied to a infinite vector in $\ell^1_\nu$. If we do so, it can be proved that all lines of this infinite matrix are the same, shifted to be always centered on the diagonal, and in this case, in which $\hat{x}$ has finite number of non-zero modes, the matrix has just a finite number of non-zero off-diagonals, we will call this non-zero elements 
%$$y_{lj}:=D_jH_l(\hat{x}),$$
%
%Let us consider that for $l=M+1,\dots,M+N$, that is for $H_l:\ell^1_\nu\rightarrow \ell^1_\nu$, we can compute

%\red{Perhaps a graphical representation of $AB$?}

% Recalling that $H=(G,F)^T$, and focusing on $F$ given by~\eqref{F} for the moment (these arguments can be easily extended to $G$ \red{JB: is this true?}), we compute,  for $n,m=M+1,\dots,M+N$
% \begin{align*}
% D_mH_n(\emb\hat{x}) &=D_m\left( -\imag\boldsymbol{k}(x_n) + \sum_{d\in D_n} f^n_d (x)^d\right)({\emb\hat{x}})\\
% &=\delta_{mn}(-\imag\boldsymbol{k}) +D_m \hat f_n(\emb \hat x)%\underbrace{\sum_{d\in D_n} f^n_d d_m(\emb \hat{ x})^{(d-e_m)}}_{D_mQ_n(\emb\hat{x})}
% \end{align*}
% %Since $\hat{x}$ has a finite number of modes, the only element with infinite number of modes in $DH(\emb\hat{x})$ is $-\imag n(1)_n$, that is cancelled out by the diagonal of $A^\dagger$, therefore the difference $A_{lj}^\dagger - D_jH_l(\emb\hat{x})$ is a matrix of the form
% while remembering the notation for the polynomial part of $F$
% $$
% (\hat f_n(x))_k= \sum_{d\in D_n} f_d^n \left( x^d\right)_k.
% $$
% By the definition of $A^\dagger$, the term $\delta_{mn}(-\imag\boldsymbol{k})$  always  cancels exactly  when computing $A^\dagger-DH(\emb\hat{x})$, and for the same reason also the finite part of  $D_m\hat f_n(\emb\hat{x})$ cancels out, leading to %, leaving us with only an infinite part that we can call the tail.
% $$
% \sup_{c\in B_r(0)} \|[A(A^\dagger-DH(\emb\hat{x}))c]_n\| = \sup_{c\in B_r(0)} \|[A(\Pi_K D\hat f(\emb\hat{x})\Pi_K-D\hat f(\emb\hat{x}))c]_n\|,
% $$
% where $D\hat f(\emb\hat x)$, being constituted of convolutions, is a  linear operator with bandwidth at most $k_1 = K(|D|-1)$ and each off-diagonal takes always the same value, as discussed in \eqref{??conv_matrix}.
% %This means that, aside from a finite $K\times K$ operator,
% Defining the operator
% $B = (\Pi_K DQ(\emb\hat{x})\Pi_K-DQ(\emb\hat{x}))$ , the structure of $DQ$ extends to $B$, therefore $B$
% has bandwidth at most $k_1$  and in the tail of $B$, each diagonal has constant value.
% Furthermore, the $K\times K$ center of $B$ is identically zero, i.e. $\Pi_K B\Pi_K = 0$.
%
% \red{TO BE DISCUSSED: what is going on here?}
%
% Considering that $A$ splits in a $K\times K$ finite part and an infinite diagonal tail, we can apply twice Lemma \ref{conv_dim} to obtain
% \begin{multline*}
% A B = A (\Pi_{2K|D|} B \Pi_{K|D|} + I_{2K|D|} B  I_{K|D|}) =\\= \Pi_{2K|D|} A \Pi_{2K|D|} B \Pi_{K|D|}  + I_{2K|D|} \imag \boldsymbol{K}^{-1} I_{2K|D|} B  I_{K|D|},
% \end{multline*}
% via multiplication of the tail of $\boldsymbol{K}^{-1}$ with a tail with a finite bandwidth, as in  \eqref{??conv_matrix}, each submatrix $(AB)_{nm}$  of $AB$, for $n,m=M+1,\dots,M+N$ here presented has the structure described in Lemma \ref{lem:weird_matrix}, therefore applying Lemma \ref{lem:weird_matrix} and Lemma \ref{operator_norm_lemma}, we can compute the norm of $AB$ exactly.
%
%
%
%
%
%
%
%
%
%
%
%
%
% %We can view $D_jQ_l(\emb\hat{x})$  as an element in $(\ell^1_\nu)^*$, and by introducing $y_{lj}=-D_jQ_l(\emb\hat{x})$, we can remark that $y_{lj}$ has just a finite number of non-zero elements, in particular, $(y_{lj})_k$ will be zeros for $|k|>K\cdot (|D|-1)$, with $K$ the number of modes of $\hat{x}$ and $|D|$ the highest power of the vector field $F$. That means that we can view  $y_{lj}\in\mathbb{C}^{2K\cdot (|D|-1)+1}$ embedded in $(\ell^1_\nu)^*$. Using this notation, we can then write the form of  the operator $A_{lj}^\dagger-D_jH_l(\emb\hat{x})$,
% %%Moreover, since for the finite part $A^\dagger$ is defined equal to $DH(\hat{x})$, the matrix $A_{lj}^\dagger-D_jH_l(\hat{x})$ has a special form
% %$$
% %\left(A_{lj}^\dagger-D_jH_l(\emb\hat{x})\right)_{mn}= \begin{cases}
% %0 & \text{if } |m|,|n|<K,\\
% %0 & \text{if } |m-n| >K\cdot (|D|-1),\\
% %(y_{lj})_{m-n} & \text{otherwise},
% %\end{cases}
% %$$
% %%with the notation $y_{lj}=D_jH_l(\hat{x})-\delta_{jl}(-\imag\tilde{1}) =\sum_{d\in D} (f_l)_d d_j \hat{ x}^{(d-e_j)}$ and t
% %%where we denoted by $|D|$ the maximum degree of the problem.
% %that could be visualized as an infinite matrix with the structure\vspace{0.2cm}
% %
% %\begin{center}
% %\begin{tikzpicture}
% %\node at (-3.7,0){$A_{lj}^\dagger-D_jH_l(\emb\hat{x})=$};
% %
% %\foreach \x in {-4,-3,-2,-1,-0,1,2,3}
% %    \filldraw[fill=black!20!white, postaction={path fading=north, fading angle=-45, fill=black!5!white}, draw=black](1+0.5*\x , 1.4- 0.5*\x) rectangle(0.5+0.5*\x,-0.9-0.5*\x);
% %\foreach \x in {-4,-3,-2,1,2,3}
% %    \node at (0.75+0.5*\x, 0.3-0.5*\x) {$y_{lj}$};
% %
% %\foreach \x in {0,-1}
% %    \node at (0.75+.5*\x, -0.4-1.7*\x) {$y_{lj}$};
% %
% %\filldraw[white, draw=black] (0,0) rectangle (1,1);
% %\node at (0.5,0.5) {0};
% %\draw[red,very thick] (0,-0.9) rectangle (1,1.9);
% %\node at (0.75,1.6) {0};
% %\node at (0.25,-0.6) {0};
% %
% %\draw[loosely dotted, very thick] (-1.6,2.5)--(-2,2.8);
% %\draw[loosely dotted, very thick] (2.9,-1.5)--(2.5,-1.2);
% %
% %\draw[very thick]  (-2, 3.4)-- (-2.1,3.4) -- (-2.1,-2.5)--(-2,-2.5);
% %\draw[very thick]  ( 2.9, 3.4)-- ( 3,3.4) -- ( 3,-2.5) -- (2.9,-2.5);
% %
% %\end{tikzpicture}
% %\end{center}
% %%
% %%blabla
% %%
% %%
% %%\begin{tikzpicture}
% %%\begin{scope}[shift={(6.5,-0.2)},scale=1]
% %%
% %%
% %%\draw[very thick]  (-5.3, 2.1)-- (-5.4,2.1) -- (-5.4,-2.1)--(-5.3,-2.1);
% %%\draw[very thick]  ( 4.5, 2.1)-- ( 4.6,2.1) -- ( 4.6,-2.1) -- (4.5,-2.1);
% %%
% %%\node at (-7,0){$A_{lj}^\dagger-D_jH_l(\hat{x})=$};
% %%\node at (4.75,0){,};
% %%
% %%\foreach \x in {-4,-3,-2,-1,-0,1,2,3}
% %%    \draw (-2+0.8*\x ,-0.4*\x) rectangle(2+0.8*\x,-0.4-0.4*\x);
% %%\foreach \x in {-4,-3,-2,-1}
% %%    \node at (-0.3+0.8*\x, -0.2-0.4*\x) {$y_{lj}$};
% %%\foreach \x in {-0,1,2,3}
% %%    \node at (+0.3+.8*\x, -0.2-0.4*\x) {$y_{lj}$};
% %%
% %%\filldraw[white, draw=black] (-0.8,-0.4) rectangle (0,0.4);
% %%\node at (-0.4,0) {0};
% %%\node at (-2.4,-0.16) {0};
% %%\node at (1.6,0.17) {0};
% %%\draw[red,very thick] (-2.8,-0.4) rectangle (2,0.4);
% %%
% %%\draw[loosely dotted,very thick] (-3.9,2) -- (-3.5,1.7);
% %%\draw[loosely dotted,very thick] (3.3,-1.7) -- (3.7,-2);
% %%
% %%\end{scope}
% %%\end{tikzpicture}
% %
% %\noindent where the red box indicates the finite part, from now on drawn shaded, with $2K|D|+1$ rows and $2K+1$ columns.
% %
% %Therefore, the matrix $A_{lj}^\dagger -D_jH_l(\emb\hat{x})$ has a finite known part and a constant known tail.
% %Once multiplied to the left with $A_{il}$, we can have two possible outcomes. Either $l\neq i$, and $A_{il}$ has just a finite part, therefore leading the product $B_{ilj}=A_{il}\left[ A^\dagger -DH(\emb\hat{x})\right]_{lj}$ to be finite, or, for $l=i$, $A_{ll}$ has a decreasing tail. In this case, the structure of the product $ A_{ll}\left[ A^\dagger -DH(\emb\hat{x})\right]_{lj}$ can be viewed  as in Figure \ref{fig_prod_B}.
% %%\begin{align*}
% %%A_{ll}\left[ A^\dagger -DH(\hat{x})\right]_{lj}&=
% %%\begin{bmatrix}
% %%\ddots\\
% %%&-\frac{1}{\imag n (x_l)_n} &\\
% %%&&A^{(F)} _{ll}&\\
% %%&&& -\frac{1}{\imag n(x_l)_n} \\
% %%&&&&\ddots
% %%\end{bmatrix}
% %%\begin{bmatrix}
% %%\ddots &\\
% %%& y_{lj}&\\
% %%&&\left[ A^\dagger -DH(\hat{x})\right]_{lj}^{(F)}&\\
% %%&&&y_{lj} &\\
% %%&&&&\ddots&\\
% %%\end{bmatrix}\\
% %%&= \begin{bmatrix}
% %%\ddots &\\
% %%& -y_{lj}\frac{1}{\imag n(x_l)_n} &\\
% %%&&A^{(F)} _{ll}\left[ A^\dagger -DH(\hat{x})\right]_{lj}^{(F)}&\\
% %%&&&-y_{lj}\frac{1}{\imag n(x_l)_n} &\\
% %%&&&&\ddots&\\
% %%\end{bmatrix},\\
% %%\end{align*}
% %
% %\begin{figure}
% %\begin{center}
% %\begin{tikzpicture}
% %
% %%\node(equal) at (-3.5,0.75){$A_{ll}\left[ A^\dagger -DH(\hat{x})\right]_{lj}=$};
% %
% %
% %\filldraw[black!5!white, draw=black] (0,0) rectangle (1.5,1.5);
% %\node[](center) at (0.75,0.75){$A_{ll}^{(F)}$};
% %
% %
% %\draw[very thick]  (3.1,-1.7) -- (3.2,-1.7)--(3.2,3.2) --(3.1,3.2);
% %\draw[very thick]  (-1.5,-1.7) -- (-1.6,-1.7)--(-1.6,3.2) --(-1.5,3.2);
% %
% %\foreach \x in {0}
% %    \draw (1.5+\x ,-\x) rectangle(2.5+\x,-1-\x);
% %\foreach \x in {0}
% %    \node[](formula) at (2+\x,-0.5-\x){$\frac{-1}{\imag n}$};
% %
% %\foreach \x in {0}
% %    \draw (-\x ,1.5+\x) rectangle(-1-\x,2.5+\x);
% %\foreach \x in {0}
% %    \node[] at (-0.5-\x,2+\x){$ \frac{-1}{\imag n}$};
% %
% %\draw[loosely dotted,very thick] (2.6,-1.1) -- (3.1,-1.6);
% %\draw[loosely dotted,very thick] (-1.1,2.6) -- (-1.6,3.1);
% %%\draw[loosely dotted,very thick] (4.6,-3.1) -- (5.1,-3.6);
% %%\draw[loosely dotted,very thick] (-3.1,4.6) -- (-3.6,5.1);
% %
% %
% %
% %\begin{scope}[shift={(6.5,0.3)},scale=0.9]
% %
% %\foreach \x in {-4,-3,-2}%{1,2,3}
% %    \draw (0.5*\x , 1.4- 0.5*\x) rectangle(-0.5+0.5*\x,-0.9-0.5*\x);
% %\foreach \x in {1,2,3}
% %    \draw (0.9+1.5+0.5*\x , 1.4- 0.5*\x) rectangle(0.9+2+0.5*\x,-0.9-0.5*\x);
% %\foreach \x in {-4,-3,-2}%1,2,3}
% %    \node at (-0.25+0.5*\x, 0.3-0.5*\x) {$y_{lj}$};
% %\foreach \x in {1,2,3}
% %    \node at (0.9+1.75+0.5*\x, -0.5*\x) {$y_{lj}$};
% %
% %\foreach \x in {0,-1}
% %    \node at (0.75+.5*\x, -0.4-1.7*\x) {$y_{lj}$};
% %
% %\filldraw[black!5!white, draw=black] (-1,-0.9) rectangle (2.9,1.9);
% %%\node at (0.75,1.6) {0};
% %%\node at (0.25,-0.6) {0};
% %\node at (0.95,0.5) {$\Pi_K\left[A^\dagger-DH(\emb\hat{x})\right]_{lj}$};
% %
% %\draw[loosely dotted, very thick] (-2.6,2.5)--(-3,2.8);
% %\draw[loosely dotted, very thick] (0.9+3.6,-1.6)--(0.9+4,-1.9);
% %
% %\draw[very thick]  (-3, 3.4)-- (-3.1,3.4) -- (-3.1,-2.5)--(-3,-2.5);
% %\draw[very thick]  ( 0.9+4.1, 3.4)-- (0.9+ 4.2,3.4) -- ( 0.9+4.2,-2.5) -- (0.9+4.1,-2.5);
% %
% %\end{scope}
% %\end{tikzpicture}
% %\begin{tikzpicture}[scale=0.9, transform shape]%[scale=0.970]
% %
% %\node() at (-4.3,0.6) {=};
% %
% %\foreach \x in {-4,-3,-2}
% %    \draw (1.8+1.05*\x , 1.4- 0.5*\x) rectangle(1.8+-1.05+1.05*\x,-0.9-0.5*\x);
% %\foreach \x in {1,2,3}
% %    \draw (-1.05+1.2+1.05*\x , 1.4- 0.5*\x) rectangle(-1+2.2+1.05*\x,-0.9-0.5*\x);
% %
% %\foreach \x in {-4,-3,-2}
% %    \node at (1.4+-0.25+1*\x, 0.3-0.5*\x) {$-y_{lj}\frac{1}{\imag n}$};
% %\foreach \x in {1,2,3}
% %    \node at (-1.05+1.75+1.05*\x, -0.5*\x) {$-y_{lj}\frac{1}{\imag n}$};
% %
% %%\foreach \x in {0,-1}
% %%    \node at (0.75+.9*\x, -0.4-1.7*\x) {$-y_{lj}\frac{1}{\imag n}$};
% %
% %\filldraw[black!5!white, draw=black] (-0.3,-0.2) rectangle (1.2,1.2);
% %\node at (0.5,0.5) {$B_{llj}^{(F)}$};
% %
% %\draw[loosely dotted, very thick] (-3.6,2.5)--(-4,2.8);
% %\draw[loosely dotted, very thick] (4.6,-1.6)--(5,-1.9);
% %
% %\draw[very thick]  (-4, 3.4)-- (-4.1,3.4) -- (-4.1,-2.5)--(-4,-2.5);
% %\draw[very thick]  ( 5, 3.4)-- ( 5.1,3.4) -- ( 5.1,-2.5) -- (5,-2.5);
% %
% %\node() at (5.7,0.5) {$=B_{llj}$};
% %
% %\end{tikzpicture}
% %\caption{The shape the product $B_{llj}=A_{ll}\left[ A^\dagger -DH(\emb\hat{x})\right]_{lj} $ is presented here,  where the apex $(F)$ was used to indicate a finite known matrix and $n$ is the index of the column. We point out in particular that constructing the matrix $B_{llj}^{(F)}$ require a finite and known number of computations. With the help of Figure \ref{figure_Z1}, we can state that the dimensions of $B_{llj}^{(F)}$ are $4K(|D|-1)+1 \times 2K(|D|-1) +1$, where $|D|$ is the maximum degree of the vector field and $K$ are the number of modes we are considering. }\label{fig_prod_B}
% %\end{center}
% %\end{figure}
% %\begin{center}
% %\begin{tikzpicture}[scale=0.6]
% %
% %%\filldraw[black!5!white, draw=black] (4.2,-1.2) rectangle (-4.2,1.2);
% %%\foreach \x in {-5,-4,-3,-2,-1,0,1,2,3,4,5}
% %%	\foreach \y in {\x -3 ,\x-2,\x-1,\x,\x+1,\x+2,\x+3}
% %%		 \draw (\x,-\y) node {\textbullet};
% %%\foreach \x in {-5,-4,-3,-2,-1,0,1,2,3,4}
% %%	\draw[dotted,thin,draw=gray] (\x,-\x)--(\x+1,-\x-1);
% %%\filldraw[white] (1.2,-1.2) rectangle (-1.2,1.2);
% %%\draw[dotted] (1.2,-1.2) rectangle (-1.2,1.2);
% %%\draw[black] (4.2,-1.2) rectangle (-4.2,1.2);
% %%\draw[red,<->] (-4.5,-1.2)--(-4.5,1.2);
% %%\draw[green,<->] (-1.3,-1.5)--(-4.2,-1.5);
% %%\draw[red,<->] (-1.1,-1.5)--(1.1,-1.5);
% %%\draw[green, <->] (1.3,-1.5)--(4.2,-1.5);
% %
% %
% %
% %\end{tikzpicture}
% %\end{center}
% %\begin{figure}
% %\begin{tikzpicture}[scale=0.3]
% %\draw [thick,black ] (-22.2+0.1,22.5-15) --(-22.6,22.5-15) -- (-22.6,7-15.4)--(-22.1,7-15.4);
% %\draw [thick,black ] (-7.1+0.2,22.5-15) --(-6.4,22.5-15) -- (-6.4,7-15.4)--(-6.9,7-15.4);
% %
% %
% %
% %\foreach \x in {-7,-8,-9,-10,-11,-12,-13,-14,-15,-16,-17,-18,-19,-20,-21,-22}
% %	\draw (\x,-\x-15) node {\textbullet};
% %
% %\filldraw[black!5!white, draw=black] (-12.5,1.5) rectangle (-16.5,-2.5);
% %
% %\foreach \x in {-13,-14,-15,-16}
% %	\foreach \y in { -1,0,1,2}
% %		 \draw (\x,-\y) node {\textbullet};
% %
% %\filldraw[black!2!white, draw=red,shift={(1.5,0)}] (-5.5,-6.5) rectangle (3.5,6.5);%(-4.5,-6.5) rectangle (2.5,5.5);
% %
% %\foreach \x in {-5,-4,-3,-2,-1,0,1,2,3,4,5,6}
% %	\foreach \y in {\x-2,\x-1,\x,\x+1,\x+2}
% %		 \draw (0.5+\x,-\y) node {\textbullet};
% %
% %\draw[thick, black] (-5,22.5-15)--(-5.5,22.5-15)--(-5.5,7-15.4)--(-5,7-15.4);
% %\draw[thick, black,shift={(1,0)}] (5.8,22.5-15)--(5.8+0.5,22.5-15)--(5.8+0.5,7-15.4)--(5.8,7-15.4);
% %
% %\draw(8.5,-0.5) node {=};
% %
% %\begin{scope}[shift={(16,0)}]
% %
% %\filldraw[black!2!white, draw=red] (-5.5,-6.6) rectangle (3.6,6.5);
% %\filldraw[green!7!white,draw=green] (-4.6,-6.4) rectangle (3.5,5.5);
% %\filldraw[black!5!white, draw=black] (-4.4,-2.5) rectangle (3.4,1.5);
% %
% %\foreach \x in{-6,-5,-4,-3,-2,-1,0,1,2,3,4,5}
% %	\foreach \y in {\x -3 ,\x-2,\x-1,\x,\x+1}
% %		 \draw (\x,-\y) node {\textbullet};
% %\foreach \x in{-4,-3,-2,-1,0,1,2,3}
% %	\foreach \y in { -2,-1,0,1}
% %		 \draw (\x,\y) node {\textbullet};
% %
% %\draw[thick, black,shift={(-1,0)}] (-5,22.5-15)--(-5.5,22.5-15)--(-5.5,7-15.4)--(-5,7-15.4);
% %\draw[thick, black,shift={(0.5,0)}] (4.5,22.5-15)--(4.5+0.5,22.5-15)--(4.5+0.5,7-15.4)--(4.5,7-15.4);
% %\end{scope}
% %\end{tikzpicture}
% %\caption{In this picture we can see the shapes of the matrices we are dealing with. The first if the matrix $A_{ll}$, where $A^{(F)}_{ll}$ has been highlighted, the second is the shape of $A^\dagger-DH(\emb\hat{x})$ (without considering the zero elements inside this shape), the third is their product. We can see how the product has an infinite number of columns that are equal up to a decreasing constant and a  center computed numerically, highlighted in grey, the result of the product with $A^{(F)}_{ll}$. Since the norm introduced in Eq. \eqref{operator_norm} just consider the columns, we are interested in computing the norm of the matrix highlighted in red, in order to consider all the elements derived from $A^{(F)}_{ll}$ and once the biggest column, using Lemma \ref{operator_norm_lemma}. In green we see $B_{llj}^{(F)}$. } %In grey are all the elements in the product matrices deriving from the elements in $A^{(F)}_{ll}$.}
% %\label{figure_Z1}
% %\end{figure}
% %
% %We remark that the tail of $B_{llj}$ is strictly decreasing, since it consists of the same vector $y_{lj}$ divided by the increasing  index $n$.  Therefore the structure of this matrix is the one required for the application of Corollary \ref{weird_matrix}, allowing us to compute $\|B_{ilj}\|$ for all values of the indices. Therefore, we can compute $Z_1$ thanks to
% %%This shows how the structure of the final matrix can be used to compute the norm of the infinite tail, with the help of Corollary \ref{weird_matrix}.
% %%Once multiplied this matrix by $A_{kl}$, we recover the same structure as presented in Corollary \ref{weird_matrix}.
% %%
% %%
% %%We can then calculate
% %\begin{multline}
% %\sup_{c\in B_r(0)} \|[A(A^\dagger-DH(\emb\hat{x}))c]_i\| \leq \sum_{j=1}^{M+N} \left\|  \sum_{l=1}^{M+N} A_{il}\left[ A^\dagger -D{H}(\emb\hat{x})\right]_{lj} \right\|_\nu r=\\
% %= \sum_{j=1}^{M+N} \left\|  \sum_{l=1}^{M+N} B_{ilj} \right\| _\nu r= Z_{1i}r.
% %\end{multline}
% %
% %
% %\tocheck{say something about the computation of the finite part as well}

\subsubsection{The $Z_2$ bound}
\label{Z_2_non_cont}


The last bound is defined as satisfying
$$
{\tilde{Z}_{2n}(r)}\geq { \sup_{b,c\in B_r(0)} \|[A(DH(\emb\hat{x}) - DH(\emb\hat{x}+b))c ]_n\|}.
$$
We apply the mean value theorem in Banach spaces:%, therefore bringing us to
\begin{align*}
\sup_{b,c\in B_r(0)}&\left\|\left(A[D{H}(\emb\hat{x})-D{H}(\emb\hat{x}+b)]c\right)_n\right\| \\
&\leq \sup_{\bar b,\bar c\in B_1(0)}\sup_{\bar{z}\in B_1(0)} \left\| \left[ A \, DD{H}(\emb\hat{x}+\bar{z}r)\bar{b}\bar{c}\right]_n\right\|r^2\\
&\leq
\sup_{\bar b,\bar c\in B_1(0)}\sup_{\bar{z}\in B_1(0)} \sum_{m=1}^{M+N} 
\left\| A_{nm}\right\|_{B(X_n,X_m)} \left\| \left[DD{H}_m(\emb\hat{x}+\bar{z}r)\bar{b}\bar{c}\right]\right\|r^2,
\end{align*}
with $\bar{b}r=b$ and $\bar{c}r=c$. The spaces $X_n$ are defined in~\eqref{e:defXn}, and the operator norms $\left\| A_{nm}\right\|_{B(X_n,X_m)}$ can computed directly (the ones on the diagonal tail, i.e.~$n=m=M+1,\dots,M+N$, by using Lemma~\ref{lem:weird_matrix}).  The bound on 
\[
  \left\| \left[DD{H}_m(\emb\hat{x}+\bar{z}r)\bar{b}\bar{c}\right]\right\|
\]
depends on $r$, but to simplify the computation we simply bound $r$ a priori by some $\rstar$, which in practice we choose to be large enough to safely assume it bigger than the validation radius. The inequality $\rstar \geq r_{\max}$ for the interval of validation $\II=(r_{\min},r_{\max})$ is checked at the end of the validation procedure.

We are thus looking for a bound on 
\begin{equation}\label{e:DDHm}
\sup_{\bar b,\bar c\in B_1(0)}\sup_{z\in B_{\rstar}(0)}  \left\| \left[DD{H}_m(\emb\hat{x}+z)\bar{b}\bar{c}\right] \right\| .
\end{equation}
We start with $m=1,\dots,M$. Both the phase condition and contination equation are linear, hence $DDH_m=0$ for $m=1,2$. For $m=3,\dots,M$ the only non-vanishing terms in the derivative are 
\[
   D^{e_n}D^{e_{n'}} H_m (\emb\hat{x}+z) = D^{e_n+e_{n'}} \tilde{g}_{m-2} (\hat{\lambda}+z_\lambda)
   \qquad\text{for } n,n' =1,\dots M.
\]
where we have written $z=(z_\lambda,z_v)$. Each of these can be bounded uniformly for $z \in B_{\rstar}(0)$ by using an interval arithmetic evaluation 
\[
   \IQ_{n,n',m} = |D^{e_n+e_{n'}}\tilde{g}_{m-2} (\hat{\lambda}_{\rstar})|
\] 
where $\hat{\lambda}_{\rstar}$ is the product of intervals $\prod_{j=1}^M [\hat{\lambda}_j-\rstar,\hat{\lambda}_j+\rstar]$. Hence, for $m=1,\dots,M$ the expression~\eqref{e:DDHm} is bounded by
\[
  \mathcal{Z}_m := \begin{cases}
  0 & \text{for } m=1,2\\
   \displaystyle\sum_{n,n'=1}^{M} \max \IQ_{n,n',m} & \text{for } m=3,\dots,M.
   \end{cases}
\]

Next we consider $m=M+1,\dots,M+N$, for which we have 
\begin{alignat}{1}
   D^{e_n}D^{e_{n'}} H_m (\emb\hat{x}+z) &= 
   \hf^{e_n+e_{n'}}_{m-M} (\emb\hat{x}+z) 
	\nonumber\\
   & \hspace*{-2cm}= \sum_{\beta \in \mathcal{D}(e_n+e_{n'},m-M)} 
	\tilde{f}_{\beta,e_n+e_{n'},m-M} (\hat{\lambda}+z_\lambda)
	 \prod_{i=1}^N (\emb\hat{v}_i+ (z_v)_i)^{\beta_i},
	 	\label{e:DenDen}
\end{alignat}
where we have used the identification (of derivatives) based on convolution multiplication introduced in Remark~\ref{r:identificationmultiplication}. We estimate these convolution polynomials term by term with the help of the Banach algebra property~\eqref{e:Banachalgebra}. Each monomial in~\eqref{e:DenDen} is bounded in norm by
\[
 \tilde{\IQ}_{\beta,n,n',m} :=
 \bigl| \tilde{f}_{\beta,e_n+e_{n'},m-M} (\hat{\lambda}_{\rstar}) \bigr|  
 \prod_{j=1}^N \bigl( \| \hat{v}_j\|_\nu + \rstar \bigr)^{\beta_j},
\] 
which is to be evaluated in an interval arithmetic sense. Using once again the Banach algebra property and the triangle inequality, this leads to the following bounds on~\eqref{e:DDHm} for $m=M+1,\dots,M+N$:
\[
  \mathcal{Z}_m = \sum_{n,n'=1}^{M+N} 
  \sum_{\beta\in \mathcal{D}(e_n+e_{n'},m-M)} 
  \max   \tilde{\IQ}_{\beta,n,n',m}.
\]
Finally, we set $\tilde{Z}_{2n} (r) := Z_{2n} r^2$ with
\[
  Z_{2n} := \sum_{m=1}^{M+N}  \left\| A_{nm}\right\|_{B(X_n,X_m)}
  	 							\mathcal{Z}_m.
\]

\subsection{Conclusion}

Once we have computed all the bounds in this section, we construct the radii polynomials%it is possible to compose the radii polynomials as
$$
p_n(r)=Y_n+(Z_{0n}+Z_{1n}) r -r +Z_{2n}r^2.
$$
%Let us remark that, being $p_n$ a second order polynomial, the zeros of $p_n$ can be computed straightforwardly. 
If there exists an $r \leq \rstar$ for which all $p_n$ are negative, then applying  Theorem~\ref{radii_bound} guarantees the existence of a fixed point contraction and, therefore, of a periodic orbit satisfying the error bounds listed in  Remark~\ref{r:errorbound}. The proof of injectivity of $A$ is discussed in Section~\ref{s:injectivity} in the more general context of continuation.


An advantage of using the mean value theorem in Section~\ref{Z_2_non_cont} is that, irrespective of the order of the vector field, the radii polynomials are always of order 2. The approach taken in, for example, \cite{castelli} and \cite{hungria-lessard} leads to $Z_2(r)$ bounds whose order depends on the order of the vector field. Our bounds are slightly less sharp due to our central goal of universal applicability, and they remain sufficiently effective in practice.



%</bounds-single>

==> bounds.tex <==

%<*bounds>


\section{Single solution bounds for radii polynomial}
\label{s:singlebounds}

For ease of exposition, we will first treat the case of a single solution.
%, i.e. we construct the bounds for the radii polynomials for $\hat x = \hat x_\s$ solution of $H_\s$ for $\s = 0,1$. 
This may also be interpreted as finding the bounds required for the $\s$-independent version of Theorem \ref{t:rad_poly}, i.e., the case where $\hat x_0 =\hat x_1$ and $\hat q_0 = \hat q_1$. We note that although the arguments below are self-contained, some additional details can be found in~\cite{BLQ}.

\subsection{$Y$ bound}\label{ss:Y_ext}

The $Y$ bound is an upper bound to
$$
\|T(\hat x) - \hat x \|_X = \|AH(\hat x)\|_X.
$$
By construction, $\hat x $ has $K$ non-zero modes. Furthermore, $F_1$ and $F_2$ are the sum of linear terms and second order convolutions. Thus $F_i(\hat x) = \Pi_i^{(2K)}F_i(\hat x)$ for $i = 1,2$, and as a consequence $ H(\hat x ) = \Pi^{(2K)}H(\hat x )$. We know that $A$ is eventually diagonal of center dimension $K$ and Remark \ref{l:sizeAy} can be applied. Therefore $AH(\hat x)$ has $2K$ non-zero modes. Thus, its norm can be computed directly with a finite number of computations in interval arithmetic.

\subsection{$Z$ bound}
The $Z$ bound presented in \eqref{e:Z_bound} can be split into three parts by considering
\begin{align*}
\begin{split}
 D T (\hat x + r b) rc = &\left[(I -AA^\dagger) + A(A^\dagger -DH(\hat x )) % \right.
%  \\&\left.
 + A(DH(\hat x )- DH(\hat x + r b)) \right]rc,
 \end{split}
\end{align*}
and computing their bounds separately. We write
\begin{equation}\label{e:split_Z}
Z(r) = Z_0r + Z_1r + Z_2(r)r
\end{equation}
with
\begin{equation}\label{Z0_bound}
Z_0 \geq \| I -AA^\dagger\|_{B(X,X)},
\end{equation}
\begin{equation}\label{Z1_bound}
Z_1 \geq \|A(A^\dagger -DH(\hat x ))\|_{B(X,X)},
\end{equation}
and
\begin{equation}\label{Z2_bound}
Z_2(r) \geq \| A(DH(\hat x )- DH(\hat x + r b))\|_{B(X,X)},
\end{equation}
where $I\in B(X,X)$ is the identity operator. 
%In the following, we will split the computation of the $Z$ into the computation of $Z_0$, $Z_1$ and $Z_2(r)$. 

\subsection{$Z_0$ bound}\label{ss:Z0_extrema}
In the case at hand, the $Z_0$ bound is fairly simple, because $A$ and $A^\dagger$ are eventually diagonal operators of center dimension $K$. Thus, applying the triangle inequality we have
$$
\| I - A A^{\dagger}\|_{B(X,X)} =
\| I \Infty - A^I A^{\dagger I}\Infty\|_{B(X,X)}+
\| I \Proj - A^F A^{\dagger F}\|_{B(X,X)}.
$$
We remark that, by definition,  the tails of the operator $A$ and $ A^\dagger$ are exact inverses  of one another. Therefore, the tail of $A^I A^{\dagger I}$ is the identity, and the first norm is zero.

 We are  left to compute
$$
\| I \Pi^{(K)} - A^F A^{\dagger F}\|_{B(X,X)}.
$$
The matrix representations of $A^F$ and $A^{\dagger F}$ are known and finite. Hence we can  compute this norm applying Equation \eqref{e:split_op_norm} and the definition of the operator norms in \eqref{e:sub_norm}.

\subsection{$Z_1$ bound}\label{ss:Z1_extrema}
In the computation of the $Z_1$ bound, the subtraction $DH(\hat x) -A^\dagger$ gives an operator  where most terms cancel and which acts as a convolution. We can represent it as
\begin{align}\label{B}
B &= DH(\hat x) -A^\dagger\nonumber\\&=   \begin{pmatrix}
 0& 0& 0\\
 0& \K b_{22}& 0\\
\K b_{31}& \K b_{32}& \K b_{33}\\
\end{pmatrix}  - \Proj \begin{pmatrix}
 0& 0& 0\\
 0& \K b_{22}& 0\\
\K b_{31}& \K b_{32}& \K b_{33}\\
\end{pmatrix}\Proj ,
\end{align}
with 
\begin{align*}
b_{22} &= 2\imag C^{\Ell}( \hat y),\\
b_{31} &= \left[ \imag ( 2\hat z* E_\ell\hat y+ \hat a ( \hat z* \hat z)),\,0,\,   \hat \lambda_1\imag ( \hat z* \hat z)\right],\\ 
b_{32} &= 2 \hat \lambda_1\imag C^{\ELL}(  \hat z)E_\ell,\\ 
b_{33} &= 2 \hat\lambda_1\imag C^{\ELL}(  E_\ell\hat y+  \hat a  \hat  z),
\end{align*}
where, with some abuse of notation,
\begin{align*}
\K b_{31} &= \K \left[ \imag ( 2\hat z* E_\ell\hat y+ \hat a ( \hat z* \hat z)),\,0,\,  \hat \lambda_1\imag ( \hat z* \hat z)\right]\\
& =\left[ \K\imag ( 2\hat z* E_\ell\hat y+ \hat a ( \hat z* \hat z)),\,0,\,  \K \hat \lambda_1\imag ( \hat z* \hat z)\right].
\end{align*}

\begin{remark}%\red{does this explain the new notation correctly?}
In the second block-row of $B$ the row corresponding to $k=0$, which was “redefined” through $\tilde{\Pi}$ to correspond to $G^{\hat{x}}_3$ rather than $(F_1)_0$, vanishes. Similar considerations hold for the the row corresponding to $j=k=0$ in the third block-row of $B$. Hence the compact notation in (7.5) may be used without including the projection $\tilde{\Pi}$. In the same way, in the rest of the paper, when the  rows corresponding to $k=0$ and $j=k=0$  vanish, we drop the use of the projection $\tilde \Pi$, such as in Equation \eqref{e:D2H} as well as for higher derivatives of $H$.
\end{remark}

We decompose 
$$
A(A^\dagger - DH(\hat x))=A^F(A^\dagger - DH(\hat x))+A^I(A^\dagger - DH(\hat x)),
$$
hence
$$
\|A(A^\dagger - DH(\hat x)\|\leq \|A^F(A^\dagger - DH(\hat x))\|+\|A^I(A^\dagger - DH(\hat x)\|.
$$
The first term has a finite number of non-zero elements, by Theorem \ref{t:size_op_prod}. The norm can  therefore be computed explicitly. The second term can be handled by computing explicitly the product $A^I B$ with the help of the two notations introduced in \eqref{e:Ai} and  \eqref{B}. Then we have
\begin{align*}
&A^I B = \\ & \begin{pmatrix}
0& 0& 0\\
0& A^I _1\K b_{22}& 0\\
A^I _2\K b_{31}&  A^I _2\K b_{32}& A^I _2\K b_{33}\\
\end{pmatrix} - 
\Proj \begin{pmatrix}
0& 0& 0\\
0& A^I_1\K b_{22}& 0\\
A^I_2\K b_{31}&  A^I _2\K b_{32}& A^I _2\K b_{33}\\
\end{pmatrix} \Proj,
\end{align*}
where the second term vanishes, and it holds that 
$$
\|A^I B\|_c \leq \begin{pmatrix}
 0& 0& 0\\
 0& \|A_1^I\K \|_{22}\|b_{22}\|_{22}& 0\\
\|A_2^I\K \|_{33}\|b_{31}\|_{31}& \|A_2^I\K \|_{33}\|b_{32}\|_{32}& \|A_2^I\K \|_{33}\|b_{33}\|_{33}\\
\end{pmatrix},
$$
with the inequality interpreted elementwise. By using Equations \eqref{e:conv_op_norm1} and \eqref{e:conv_op_norm}, we obtain
\begin{align*}
&\|b_{22}\|_{22} \leq 2\| \hat y\|_{\Ell},\\
&\| b_{31} \|_{31}\leq \max\{ \| 2\hat z* E_\ell\hat y+ \hat a ( \hat z* \hat z)\|_{\ELL},\,0,\, |\hat \lambda_1|\|  \hat z* \hat z\|_{\ELL}\},\\
& \|b_{32}\|_{32} \leq 2 |\hat \lambda_1|\|  \hat z\|_{\ELL},\\
& \|b_{33}\|_{33} \leq 2|\hat \lambda_1|\|  E_\ell\hat y+  \hat a  \hat  z\|_{\ELL},
\end{align*}
and $\|A_i^I\K\|$ for $i = 0,1$ fits the setup discussed in Section \ref{s:tail} and can be computed via \eqref{e:bound_tail}.

\subsection{$Z_2$ bound}\label{ss:Z2_extrema}

Following the approach already presented in \cite{QJBcontinuation}, for the computation of $Z_2(r)$ we can apply the  mean value theorem. We  introduce $R$, an \textit{a priori} bound on the validation radius $r^*$, and we obtain
$$
\| A( DH(\hat x) - DH(\hat x + rb)) \| _{B(X,X)}\leq \sup_{b,c \in B_1(0)} \| AD^2H(\hat x + R b)c\|_{B(X,X)}.
$$
The major difference with respect to \cite{QJBcontinuation} is that in the case at hand the norm of $D^2H(\hat x + R b)$ is not finite because it includes spatial derivative operators. Therefore, in this case the multiplication with $A$ plays a key role in keeping the $Z_2(r)$ bound finite. 
%
We start by computing $D^2H$ explicitly, using the notation introduced in~\eqref{e:notation_Xop}. We compute it at a point $x = (\lambda_1, \lambda_2, a, y, z)$ and apply it to $w =(\beta_1, \beta_2, b,  r,s)\in X$:
\begin{equation}\label{e:D2H}
D^2H(x)w =
\begin{pmatrix}
0&0&0\\
d_{21}(x,w)&
d_{22} (x,w)
&0\\
d_{31}(x,w)
&
d_{32} (x,w)
&
d_{33}(x,w) 
\end{pmatrix},
\end{equation}
with 
\begin{align*}
d_{21}(x,w)&=[0,\K^4r,0],\\
d_{22}(x,w)& = \K^4\beta_2- 2 \imag \K C^{\Ell}(r),\\
d_{31}(x,w)& =d_{311}(x,w),
\K^4(z\beta_1 +  \lambda_1 s), 
-\imag \K({\beta_1}z*z+2\lambda_1 z*s),\\
d_{311}(x,w)& = \K^4(z\beta_2+\lambda_2 s)-\K^2s
%\\ &\qquad 
-\imag \K (2E_\ell y*s+2z*E_\ell r+b z*z+2az*s),\\
d_{32} (x,w)&= -2\imag \K C^{\ELL}(\lambda_1 s + {\beta_1}z)E_\ell,\\
d_{33}(x,w) &= \K^4(\lambda_2{\beta_1}+\lambda_1{\beta_2})-\K^2{\beta_1}
\\ &\qquad
-2\imag \K C^{\ELL}(\beta_1E_\ell y+\lambda_1E_\ell r +a\beta_1z+\lambda_1(b z+as)).
\end{align*}


We notice that $D^2H$ is a $2K$-diagonal operator since it is the product of diagonal operators and convolution operators. All $d_{nm}(x,w)$ are of the form
\begin{equation}\label{e:d_jk}
d_{nm}(x,w) = \K d^{[1]}_{nm}(x,w) + \K^2d^{[2]}_{nm}(x,w) + \K^4d^{[4]}_{nm}(x,w),
\end{equation}
for $n,m= 1,\dots, 3$.

We use the notation introduced in \eqref{e:notation_Xop} to write
$$
A =  \begin{pmatrix}
A_{11} & A_{12} & A_{13}\\
 A_{21} & A_{22} & A_{23}\\
 A_{31} & A_{32} & A_{33}
\end{pmatrix}.
$$
With this notation, we can write
$$
(AD^2H(\hat x + R b)c)_{im} =  \sum_{n=1,\dots,3}A_{in} d_{nm}(\hat x + R b,c),
$$
and by the triangle inequality we can bound
$$
\|(AD^2H(\hat x + R b)c)_{im}\|_{im} \leq  \sum_{n=1,\dots,3}\|A_{in} d_{nm}(\hat x + R b,c)\|_{im} .
$$
With the notation introduced in \eqref{e:d_jk} and applying again the triangle inequality, we have
$$
\|A_{in} d_{nm}(\hat x + R b,c)\|_{im}\leq \sum_{p = 1,2,4} \||A_{in} \K^p\|_{in}\|d^{[p]}_{nm}(\hat x + R b,c)\|_{nm}.
$$
Since $K$ is a diagonal operator, it holds that, by Lemma \ref{l:eventual_diag},
$$
\| A_{ij} \K^p\|_{ij} = \max\{\|A_{ij} ^F\Proj \K^p\|_{ij},\|A^I_{ij}\Infty \K^p\|_{ij}\},
$$
where the first norm can be computed directly and the second can be estimated by applying the bounds from Section \ref{s:tail}. The norms $\|d^{[p]}_{nm}(\hat x + R b,c)\|_{nm}$ can be easily estimated for all $n$ and $m$ because they are sums and products of scalars and convolution operators, hence \eqref{e:conv_op_norm1} and \eqref{e:conv_op_norm} and the bound $\|x+Rb\|_c\leq\|x\|_c+R$ suffice to bound these terms. 

As an example we consider $d_{33}^{[p]}(x,w)$, which can be written as
\begin{align*}
d^{[1]}_{33}(x,w) &=
-2\imag  C^{\ELL}(\beta_1E_\ell y+\lambda_1E_\ell r +a\beta_1z+\lambda_1(b z+as)),\\
d^{[2]}_{33}(x,w) & = -{\beta_1},
\\
d^{[4]}_{33}(x,w) & = \lambda_2{\beta_1}+\lambda_1{\beta_2}.
\end{align*}
Using $\|x+Rb\|_c\leq\|x\|_c+R$ and $\|b\|_c \leq1$, we obtain, for any $\|w\|_X\leq 1$,
\begin{align*}
\|d^{[1]}_{33}(x+Rb,w)\|_{33} &\leq
2\left(\| y\|_{\ell}+|\lambda_1|+2R+(|a|+R)(\|z\|_{\ELL}+R)\right)\\
&\qquad\qquad+2(|\lambda_1|+R)( \|z\|_{\ELL}+|a|+2R),
\\
\|d^{[2]}_{33}(x+Rb,w) \|_{33}& \leq 1,
\\
\|d^{[4]}_{33}(x+Rb,w) \|_{33} & \leq |\lambda_2|+|\lambda_1|+2R.
\end{align*}
The estimates of the other terms are treated in an analogous manner.
 
\section{Bounds for segment validation}\label{s:cont_bound}

To compute the bounds introduced in Section \ref{s:radii_pol} that include a maximum over $s\in[0,1]$, we use the following lemma.


\begin{lemma}\label{l:s_bound}
Let $f:[0,1]\mapsto\mathbb{C}$ be $C^2$, then
\begin{equation}\label{max_s}
\max_{s\in[0,1]} |f(s)| \leq \max\{ |f(0)|,|f(1)|\} +  \dfrac{1}{8} \max_{x\in[0,1]}|f''(x)|.
\end{equation}
\end{lemma}

For the proof, we refer to \cite[Lemma~8.1]{QJBcontinuation}. We want to apply this lemma to a variety of cases. The most general application is the following.

\begin{lemma}\label{l:general_cont_bound}
Let $i,j\in\{1,2,3\}$. For $s\in[0,1]$ let $A(s):X_i\rightarrow X_j$ be a family of bounded linear operators dependent on a parameter $s$, with matrix representation $A(s) = (A_{k_1k_2}(s))_{k_1\in I_i,k_2\in I_j}$, with $I_1$ and $I_2$ the appropriate set of indices for $X_i$ and $X_j$ respectively, that is $I_1 = \{1,2,3\}, I_2 = \mathbb{Z}, I_3 = \mathbb{Z}^2$. Then
\begin{align*}
\max_{s\in[0,1]} \|A(s)\|_{ij} & \leq \left\| (\max\{ |A_{k_1k_2}(0)|,|A_{k_1k_2}(1)|\})_{k_1\in I_i,k_2\in I_j}\right\|_{ij}+  \\
& \hspace{4cm}\dfrac{1}{8} \left\|\left(\sup_{x\in[0,1]}|A''_{k_1k_2}(x)| \right)_{k_1\in I_i,k_2\in I_j}  \right\|_{ij},
\end{align*}
provided the elementwise second derivatives $A''_{k_1k_2}$ exists for all $k_1 \in I_1$ and $k_2\in I_2$ and the second term is finite.
\end{lemma}
For the proof, we refer to \cite{QJBcontinuation}. That proof is carried out on a different space but the proof on $X$ follows in the same way.

Considering the space $X$ and the linear operator $B(s):X\rightarrow X$ for $s\in[0,1]$, using the notation \eqref{e:notation_Xop}, we have
\begin{equation}\label{e:norm_max}
\max_{s\in[0,1]} \|B(s)\|_{B(X,X)} 
\leq \max_{j = 1,\dots, 3} \sum_{i = 1,\dots,3} \max_{s\in [0,1]}\| B_{ij}(s)\|,
\end{equation}
and we can apply Lemma \ref{l:general_cont_bound} to each $B_{ij}$. Having already introduced the operators $A_0$ and $A_1$, we  introduce a notation for their difference:
$$
A_\Delta = A_1-A_0.
$$
In general, the subscript $\Delta$ will indicate the difference between the element at hand at $s =1$ and $s=0$. 

\begin{remark}
By construction, $A_\Delta$ is an eventually diagonal operator of center dimension $K$, hence $A_\Delta = A^F_\Delta + A^I_\Delta$. The tail of $A_\Delta$ is non-zero in general, but applying the same notation as in \eqref{e:Ai}, it is computable element wise by
\begin{equation}\label{e:AI_Delta}
A_\Delta^I =
\begin{pmatrix}
0&0&0\\
0 & A_{\Delta 1}^I & 0\\
0 & 0 & A_{\Delta 2}^I
\end{pmatrix}\Infty.
\end{equation}
Here
$$
A_{\Delta 1}^I=P_1(1)^{-1} - P_1(0)^{-1} = \frac{P_1(0) -P_1(1) }{P_1(0) P_1(1)},
$$
and 
$$
A_{\Delta 2}^I=P_2(1)^{-1} - P_2(0)^{-1} = \frac{P_2(0) -P_2(1) }{P_2(0) P_2(1)},
$$
with 
$$
P_1(\s) \bydef   \hat \lambda_{\s 2}\K^4- \K^2, \quad\text{for } \s = 0,1,
$$
and 
$$
P_2(\s) \bydef 
\imag \J + \hat \lambda_{\s 1} \hat \lambda_{\s 2} \K^4 -  \hat \lambda_{\s 1} \K^2 ,\quad\text{for } \s = 0,1.
$$
All inverses, fractions and multiplications are here intended elementwise. %because we are working with diagonal operators.
\end{remark}

\subsection{$Y$ bound}\label{ss:Y_bound}

In the continuation case, we want to compute $Y$ such that
$$
\max_{s\in[0,1]}\| A_s H_s(\hat x_s)\|_X\leq Y.
$$
We denote $A_s H_s(\hat x_s) = (g_1(s),g_2(s),g_3(s))\in X = \mathbb{R}^3\times \Ell\times \ELL$ for $s\in [0,1]$.

In a similar way as in Lemma~\ref{l:general_cont_bound} it holds, for $i = 1,2,3$, that
\begin{align}\label{Y_bound_s}
\begin{split}
\max_{s\in[0,1]} \|g_i(s)\|_{X_i}\leq 
\frac{1}{8}&\left\|\left(\max_{s\in [0,1]}\left|g_k''(s)\right|\right)_{k\in I_i}\right\|_{X_i}\\& +
\left \| \left(\max\left\{ | ( g_i(0))_k |,| (g_i(1))_k|\right\} \right)_{k\in I_i}\right\|_{X_i}.
\end{split}
\end{align}
Applying the approach presented in Section \ref{ss:Y_ext} we can compute all nonvanishing components of $g_i(0)$ and $g_i(1)$, thus making the second term straightforward to bound explicitly. We are left with having to bound the second order derivative. It holds, by linearity in $s$ of $\hat x_s$ and $A_s$, that
\begin{align*}
g''(s) = D_sD_s(A_sH_s(\hat x_s))
& =
2A_\Delta DH(\hat x_s) x_\Delta + A_s D_sD_sH(\hat x_s)
\\  & =
 2A_\Delta DH(\hat x_s) x_\Delta + A_s DDH(\hat x_s)x_\Delta x_\Delta.
\end{align*}
By construction, $x_\Delta \in \Pi^{(K)} X$, while $DH(\hat x_s)$ acts on $x_\Delta$ as a
% second order 
convolution. Therefore $DH(\hat x_s) x_\Delta\in\Pi^{(2K)}X$. By Lemma \ref{l:sizeAy}, thanks to $A_\Delta$ being eventually diagonal of center dimension $K$, we find that $A_\Delta DH(\hat x_s) x_\Delta\in\Pi^{(2K)}X$. In the same way we can prove that  $$A_s DDH(\hat x_s)x_\Delta x_\Delta\in\Pi^{(2K)}X.$$ Thus, we can bound $\|D_sD_s(A_sH_s(\hat x_s))\|_c$ by a computation where we replace $\hat x_s$ by the \emph{interval} 
\begin{equation}\label{e:four_star}
x_s = \hat x_0 + [0,1] \cdot x_\Delta,
\end{equation}
interpreted elementwise, 
and all the computations involving $\hat x_s$ are performed using interval arithmetic. Thus, both terms in \eqref{Y_bound_s} can be bounded explicitly.

\subsection{$Z_0$ bound}\label{ss:Z0_cont}

Applying the  splitting \eqref{e:split_Z}, the $Z_{0}$ bound is such that
$$
Z_0\geq \max_s\|I-A_sA^\dagger_s\|_{B(X,X)}.
$$
Using the notation \eqref{e:notation_Xop} we apply Lemma \ref{l:general_cont_bound} to obtain, for $i,j = 1,2,3$, 
\begin{align*}
&\|(I - A_sA^\dagger_s)_{ij}\|_{ij}\leq\\
&\hspace{1.5cm} \left\| \left(\max\{ |(( I-A_0A^\dagger_0)_{ij})_{k_1k_2}|,|( (I-A_1A^\dagger_1)_{ij})_{k_1k_2}|\} \right)_{k_1\in I_1,k_2\in I_2} \right\|_{ij}\\
&\hspace{5cm}+ 
\frac{1}{4}\left\|\left(\sup_s|(A_\Delta A^\dagger_\Delta)_{ij})_{k_1k_2}|\right)_{k_1\in I_1,k_2\in I_2} \right\|_{ij}.
\end{align*}

The first term is the elementwise maximum over $ I-A_0A^\dagger_0$ and $ I-A_1A^\dagger_1$. We computed these terms and their norm separately in Section \ref{ss:Z0_extrema}. Here we simply need to take the elementwise maximum of their absolute values \emph{before} taking the norm, but it is otherwise a  straightforward extension of the computation in Section \ref{ss:Z0_extrema}.  We are left to compute $\|(A_\Delta A^\dagger_\Delta)_{ij}\|_{ij}$, where the maximum over $s$ is dropped, because the argument does not depend on $s$.  The product $A_\Delta A^\dagger_\Delta$ is the product of two eventually diagonal operator of center dimension $K$, thus it is again an eventually diagonal operator of center dimension $K$. It then holds that
$$
\| I-A_\Delta A^\dagger_\Delta\|  \leq  \max
\{ 
\| \Proj-A^F_\Delta A^{\dagger F}_\Delta \|  ,
\|  \Infty  -A^I_\Delta A^{\dagger I}_\Delta \|
\}
$$
The norm of the finite center can be computed directly, hence we will concentrate on the bound of the tail operator.

Let us recall, from the definitions of $A_i$ and $A^\dagger_i$, with $i = 0,1$, that
\begin{equation}\label{e:Adagger_Delta}
A^{\dagger I}_\Delta= A^{\dagger I}_0 - A^{\dagger I}_1 =\begin{pmatrix}
0&0&0\\
 0 & 
\hat \lambda_{2\Delta}\K^4 & 0\\
0 & 0 &
(\hat \lambda_1 \hat \lambda_2)_\Delta \K^4 -  \hat \lambda_{1\Delta}\K^2 
\end{pmatrix}\Infty,
\end{equation}
and
$
A^I_\Delta
$ is defined in \eqref{e:AI_Delta}. It follows from Equations \eqref{e:Adagger_Delta} and \eqref{e:AI_Delta} that 
$$
A^I_\Delta A^{\dagger I}_\Delta =\begin{pmatrix}
0&0&0\\
 0 & B_1 & 0\\
0 & 0 &
 B_2 
\end{pmatrix}\Infty
$$
with  
\begin{align*}
&B_1 =
\frac{( \hat \lambda_{2\Delta}\K^4)(  \hat \lambda_{2\Delta}\K^4)}{ 
( \hat \lambda_{21}\K^4- \K^2)( 
 \hat \lambda_{20}\K^4-\K^2)},\\
 &B_2 =
\frac{( (\hat \lambda_1 \hat \lambda_2)_\Delta \K^4 -  \hat \lambda_{1\Delta}\K^2)(  (\hat \lambda_1 \hat \lambda_2)_\Delta \K^4 -  \hat \lambda_{1\Delta}\K^2 ) }{ 
(\imag \J + \hat \lambda_{11}\hat \lambda_{21} \K^4 -  \hat \lambda_{11}\K^2 )( 
\imag \J + \hat \lambda_{10} \hat \lambda_{20} \K^4 -  \hat \lambda_{10}\K^2 )}.
\end{align*}
With this format, we could apply directly the results of Section \ref{s:tail}, but we prefer instead to avoid computing bounds having diagonal terms of order 8. We therefore simplify the computations by considering 
\begin{align*}
&\|  B_1 \Infty \|_{22}  \leq \left\|  
\tfrac{\hat \lambda_{2\Delta}\K^4}
{  \hat \lambda_{21}\K^4- \K^2} \Infty  \right\|_{22}  
\left\|  
\tfrac{  \hat \lambda_{2\Delta}\K^4}{ 
  \hat \lambda_{20}\K^4-\K^2} \Infty \right\|_{22}  ,\\
 &
 \|  B_2 \Infty \|_{33}  \leq \left\|   
 \tfrac{ (\hat \lambda_1 \hat \lambda_2)_\Delta \K^4 -  \hat \lambda_{1\Delta}\K^2}{
 \imag \J + \hat \lambda_{11} \hat \lambda_{21} \K^4 -  \hat \lambda_{11}\K^2} \Infty \right\|_{33}  
 \left\|   \tfrac{ (\hat \lambda_1 \hat \lambda_2)_\Delta \K^4 -  \hat \lambda_{1\Delta}\K^2 }{\imag \J + \hat \lambda_{10} \hat \lambda_{20} \K^4 -  \hat \lambda_{10}\K^2 } \Infty \right\|_{33}  .
\end{align*}
In all these four cases, we can apply the approach presented in Section \ref{s:tail} to bound the norms of the rational tail operators.

This concludes the computation of the $Z_0$ bound in the continuation setting.

\subsection{$Z_1$ bound}

Applying Lemma \ref{l:general_cont_bound}, and using the notation
$$
A_s(A^\dagger_s - DH_s(\hat x_s)) = \begin{pmatrix}
B_{11}(s) & B_{12}(s) & B_{13}(s) \\
B_{21}(s) & B_{22}(s) & B_{23}(s) \\
B_{31}(s) & B_{32}(s) & B_{33}(s)
\end{pmatrix}
$$
we can write 
\begin{multline*}
\max_{s\in[0,1]}\sup_{c\in B_r(0)} \| B_{ij}(s)\|_{ij}  \leq \\\left \| \left(\max\left\{ \left| (B_{ij}(1))_{k_1k_2} \right|,\, \left|(B_{ij}(0))_{k_1k_2}\right|\right\} \right)_{k_1\in I_1,k_2\in I_2}\right\|_{ij} \\
+ \frac{1}{8} \left\| \max_{s\in[0,1]}|(B''_{ij}(s))_{k_1k_2}|\right\|_{ij} \leq Z_{1}r,
\end{multline*}
for $i,j = 1,2,3$.
The bound at the end points, $s=0,1$, follows from the procedure presented in Section \ref{ss:Z1_extrema} taking the elementwise maxima before taking the norms, as in Section \ref{ss:Z0_cont}.  Therefore it remains to bound the components of 
$$
B''(s) = D_{s}D_s \left( A_s(A^\dagger_s-DH_s(\hat x_s))\right).
$$
By linearity of $A_s$ and $A^\dagger_s$ in $s$, it holds that
\begin{align}\label{e:Ds2Z1}
 D_sD_s &\left( A_s(A^\dagger_s-DH_s(\hat x_s))\right)&
\\&= 2(A_\Delta D_s \left( A^\dagger_s-DH_s(\hat x_s)\right)+ A_s D_{s}D_s\left(A^\dagger_s-DH_s(\hat x_s)\right)
\\ \nonumber &= 2A_\Delta A^\dagger_\Delta -  2A_\Delta D^2H_s(\hat x_s)x_\Delta  -  A_sD^3H_s(\hat x_s)x_\Delta x_\Delta.
\end{align}

We already discussed a bound for $A_\Delta A^\dagger_\Delta$ in Section \ref{ss:Z0_cont}. For the second term $A_\Delta D^2H_s(\hat x_s)x_\Delta$, we recall the direct computation of $D^2H_s$ in \eqref{e:D2H}. Furthermore, we have $\hat x_s,x_\Delta \in \Pi^{(K)}X$. Since $A_\Delta$ is an eventually diagonal operator, it holds that
$$
A_\Delta D^2H_s(\hat x_s)x_\Delta = A_\Delta ^F \Pi^{(K)} D^2H_s(\hat x_s)x_\Delta + A_\Delta^I  \Infty  D^2H_s(\hat x_s)x_\Delta.
$$
In the first term, we now replace, as in Section \ref{ss:Y_bound}, $\hat x_s$ by the interval $x_s$ defined in \eqref{e:four_star}. Since we know that $D^2H_s(\hat x_s)$ has a finite number of nonvanishing (interval) components, we can explicitly compute all the nonvanishing components of the first term and compute a bound for $\|A_\Delta ^F \Pi^{(K)} D^2H_s(\hat x_s)x_\Delta\|_c$. 
%From now on we replace $\hat x_s$ by $x_s$ whenever convenient.

For the second term, it holds that
$$
A_\Delta^I  \Infty  D^2H_s(\hat x_s)x_\Delta =   \begin{pmatrix}
0 & 0 & 0\\
0 & A^I_{\Delta 1} d_{22} (\hat x_s,x_\Delta) & 0 \\
0 & A^I_{\Delta 2} d_{32} (\hat x_s,x_\Delta)  & A^I_{\Delta 2} d_{33} (\hat x_s,x_\Delta) 
\end{pmatrix}.
$$
With the notation introduced in \eqref{e:AI_Delta}, we can write 
\begin{align*}
& A^I_{\Delta 1} d_{22} (\hat x_s,x_\Delta) =\\&\qquad\quad \frac{  \hat \lambda_{\Delta 2}\K^4}{(  \hat \lambda_{20}\K^4-\K^2)(  \hat \lambda_{21}\K^4-\K^2)}\Infty d_{22} (\hat x_s,x_\Delta) ,\\
& A^I_{\Delta 2} d_{32} (\hat x_s,x_\Delta) = \\&\qquad\quad\frac{  (\hat \lambda_1 \hat \lambda_2)_\Delta\K^4 -  \hat \lambda_{1\Delta}\K^2}{(\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2)(\imag \J + \hat \lambda_{11} \hat \lambda_{21}\K^4 -  \hat \lambda_{11}\K^2)}\Infty d_{32} (\hat x_s,x_\Delta),\\
& A^I_{\Delta 2} d_{33} (\hat x_s,x_\Delta) = \\&\qquad\quad\frac{  (\hat \lambda_1 \hat \lambda_2)_\Delta\K^4 -  \hat \lambda_{1\Delta }\K^2}{(\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2)(\imag \J + \hat \lambda_{11} \hat \lambda_{12}\K^4 -  \hat \lambda_{1 1}\K^2)}\Infty d_{33} (\hat x_s,x_\Delta).
\end{align*}
We apply a splitting of the fraction similar to the one used in Section \ref{ss:Z0_cont} to simplify the computations, thereby  retrieving 
\begin{align*}
& \|A^I_{\Delta 1} d_{22} (\hat x_s,x_\Delta)\|_{22}  =\\&\qquad\quad
\left\|\Infty
 \frac{d_{22} (\hat x_s,x_\Delta)}{  \hat \lambda_{20}\K^4-\K^2}\right\|_{22}  \left\|\Infty
\frac{   \hat \lambda_{2\Delta }\K^4}{  \hat \lambda_{21}\K^4-\K^2}\right\|_{22} ,\\
&\| A^I_{\Delta 2} d_{32} (\hat x_s,x_\Delta) \|_{32} 
= \\&\qquad\quad
\left\|\Infty \frac{d_{32} (\hat x_s,x_\Delta)}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{32} \left\|\Infty\frac{ (\hat \lambda_1 \hat \lambda_2)_\Delta\K^4 -  \hat \lambda_{1\Delta}\K^2}{\imag \J + \hat \lambda_{11} \hat \lambda_{21}\K^4 -  \hat \lambda_{11}\K^2}\right\|_{32} ,\\
&\| A^I_{\Delta 2} d_{33} (\hat x_s,x_\Delta) \|_{33} = \\&\qquad\quad
\left\| \Infty \frac{d_{33} (\hat x_s,x_\Delta)}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{33} \left\|\Infty \frac{ (\hat \lambda_1 \hat \lambda_2)_\Delta\K^4 -  \hat \lambda_{1\Delta}\K^2}{\imag \J + \hat \lambda_{11} \hat \lambda_{21}\K^4 -  \hat \lambda_{11}\K^2}\right\|_{33} .
\end{align*}
The second norm in each bound can be computed by applying the procedure presented in Section \ref{s:tail}, but the first norms are not yet in that form, because $d_{ij}(\hat x_s,x_\Delta)$ are not diagonal operators. Using the expressions for $d_{ij}$ introduced in Section \ref{ss:Z2_extrema}, we estimate\begin{align*}
&\left\|\Infty \frac{d_{22} (\hat x_s,x_\Delta)}{  \hat \lambda_{20}\K^4-\K^2}\right\|_{22}  \leq 
\\&\hspace{2.5cm}
\left\|\Infty \frac{\K^4}{  \hat \lambda_{20}\K^4-\K^2}\right\|_{22} |\lambda_{2\Delta}|+ \left\|\Infty \frac{ 2\K }{  \hat \lambda_{20}\K^4-\K^2}\right\|_{22}  \|y_\Delta\|_{\Ell}  ,
\end{align*}
and
\begin{align*}
&\left\| \Infty \frac{d_{32} (\hat x_s,x_\Delta)}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{32} \leq 
\\&\hspace{3cm}
\left\| \Infty \frac{  
2 \K}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{33}\|\lambda_{1s} z_\Delta + \lambda_{1\Delta}z_s\|_{\ELL},
\end{align*}
and
\begin{align*}
&\left\|\Infty  \frac{d_{33} (\hat x_s,x_\Delta)}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{33}  \leq 
\\&\hspace{3cm}
\left\| \Infty \frac{
\K^4
}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{33} |\lambda_{2s}\lambda_{1\Delta}+\lambda_{1s}\lambda_{2\Delta}|
\\&\hspace{3cm}
+\left\| \Infty \frac{\K^2
}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{33}  |\lambda_{1\Delta}|
\\&\hspace{3cm}
+ \left\| \Infty \frac{2 \K
}{\imag \J + \hat \lambda_{10} \hat \lambda_{20}\K^4 -  \hat \lambda_{10}\K^2}\right\|_{33} 
\\&\hspace{3cm}
+ \|(E_\ell y_s+a_sz_s)\lambda_{1\Delta}+\lambda_{1s}(a_\Delta z_s+a_sz_\Delta + E_\ell y_\Delta)\|_{\ELL}
.
\end{align*}
All these terms can either be bounded by direct interval arithmetic computation (since both $x_\Delta$ and the interval-valued $x_s \ni \hat x_s$ have finitely many nonvanishing components only) or via the bounds on rational tail operators in Section \ref{s:tail}.

We will now bound the final term in \eqref{e:Ds2Z1}, $A_sD^3H_s(\hat x_s)x_\Delta x_\Delta$. This term first requires the computation of $D^3H_s(\hat x_s)x_\Delta x_\Delta$, that is
\begin{equation*}
D^3H(\hat x_s)x_\Delta x_\Delta =
\begin{pmatrix}
0&0&0\\
0&0&0\\
d^3_{31}(\hat x_s,x_\Delta)
&
d^3_{32}(\hat x_s,x_\Delta)
&
d^3_{33}(\hat x_s,x_\Delta)
\end{pmatrix} ,
\end{equation*}
with 
\begin{align*}
d^3_{31}(\hat x_s,x_\Delta)&=\begin{bmatrix}d^3_{311}(\hat x_s,x_\Delta),
2\K^4z_\Delta{\lambda_{1\Delta}} ,
d^3_{313}(\hat x_s,x_\Delta)\end{bmatrix},
\\
d^3_{311}(\hat x_s,x_\Delta)&=2\K^4z_\Delta\lambda_{2\Delta}
-\imag \K (4E_\ell y_\Delta*z_\Delta+4a_\Delta z_\Delta*z_s+2a_sz_\Delta*z_\Delta)\\
d^3_{313}(\hat x_s,x_\Delta)&=-\imag \K(4\lambda_{1\Delta} z_\Delta*z_s+
2\lambda_{1s} z_\Delta*z_\Delta),\\
d^3_{32}(\hat x_s,x_\Delta)&= 
-4\imag \K\lambda_{1\Delta} C^{\ELL} (z_\Delta)E_\ell, \\
d^3_{33}(\hat x_s,x_\Delta)&=
2\K^4\lambda_{1\Delta}{\lambda_{2\Delta}}\\&\qquad
-4\imag \K C^{\ELL}(\lambda_{1s} a_\Delta z_\Delta +{\lambda_{1\Delta}}(E_\ell y_\Delta+a_\Delta z_s+a_sz_\Delta)).
\end{align*}
The norm of $A_sD^3H(\hat x_s)x_\Delta x_\Delta$ can be bounded by considering $A_s$ as the interval $[A_0,A_1]$, interpreted elementwise and using the triangular inequality:
$$
\|A_sD^3H(\hat x_s)x_\Delta x_\Delta\| \leq \|A_s^ID^3H(\hat x_s)x_\Delta x_\Delta\| + \|A_s^FD^3H(\hat x_s)x_\Delta x_\Delta\|.
$$
Here we can bound the finite part with Corollary \ref{l:finite_norm}, since all nonvanishing terms can be enclosed using interval arithmetic. The infinite tail  gives
$$
A_s^ID^3H(\hat x_s)x_\Delta x_\Delta = \begin{pmatrix}
0 & 0 & 0\\
0 & 0 & 0\\
0 & A^I_{s2} d^3_{32} & A^I_{s1} d^3_{33}
\end{pmatrix},
$$
and
\begin{align*}
\|A^I_{s2} d^3_{32}\|_{32} &\leq4 \|A^I_{s2} \K\|_{32}\|\lambda_{1\Delta} z_\Delta\|_{\ELL},\\
\|A^I_{s2} d^3_{33}\|_{33} &\leq 2\|A^I_{s2}\K^4\|_{33}|\lambda_{1\Delta}\lambda_{2\Delta}|
+ 4\|A^I_{s2}\K\|_{33}\|4\\ &\qquad + \lambda_{1s} a_\Delta z_\Delta +{\lambda_{1\Delta}}(E_\ell y_\Delta+a_\Delta z_s+a_sz_\Delta)\|_{\ELL}.
\end{align*}
These terms can be bounded either by direct computation or by the technique presented in Section \ref{s:tail}.

\subsection{$Z_2$ bound}
For the $Z_2$ bound in the continuation case, we proceed in the same way as in Section \ref{ss:Z2_extrema}. By applying the mean value theorem we have
\begin{align*}
&\max_{s\in[0,1]}\sup_{b,c\in B_r(0)} \left\|  A_s \left( DH_s(\hat x_s) -DH_s(\hat x_s+rb)rc\right)\right\| 
\leq\\
& \qquad\qquad\qquad \qquad\max_{s\in[0,1]}\sup_{{b},{c}\in B_1(0)}  \left\|  A_s D^2H _s(\hat x_s+R {b}){c} \right\| r^2.
\end{align*}
Following the strategy presented in Section \ref{ss:Z2_extrema} and using the convexity of the norm, we bound
\begin{align*}
&\max_{s\in[0,1]}\sup_{\bar{b},\bar{c}\in B_1(0)} \sup_{z\in B_1(0)} \left\| \left( A_s D^2H _s(\hat x_s+zr) \bar{b}\bar{c} \right)_n \right\| r^2\leq\\&\qquad\qquad
\max_{A = \{A_0,A_1\}} \sup_{\bar{b},\bar{c}\in B_1(0)} \sup_{z\in B_1(0)} \left\| \left( A D^2H_s(\hat x_s+zr) \bar{b}\bar{c} \right)_n \right\| r^2,
\end{align*}
and we can apply the same process as in Section \ref{ss:Z2_extrema} of estimating ``monomial by monomial'',  with the additional step that
$$
\| \hat x_s\|_c \leq \max\{ \|\hat x_0\|_c,\|\hat x_1\|_c\},
$$
where the component norm $\|\cdot\|_c$ is defined in \eqref{e:c_norm}.
%</bounds>

==> conclusion.tex <==
%<*conclusion>

We have until now discussed  how to validate already computed numerical solutions. Before presenting the results, we explain how the first numerical solution $\hat x = (\hat \lambda_1, \hat \lambda_2, \hat a, \hat y, \hat z)$ is computed. We consider the stationary problem \eqref{e:eq_y} projected onto a finite dimensional subset $\Proj \Ell \subset \Ell$. In this framework, Equation \eqref{e:eq_y} becomes a finite dimensional system which we can easily solve numerically for $y$ at any given $\lambda_2 = \gamma$. Then, it is straightforward to compute all the eigenvalues $(\mu_1,\dots \mu_{2K+1})$ associated to \eqref{e:eq_y} at a given $\gamma$ and $y$. This procedure does not need to be rigorous. 
We look for a value $\gamma = \lambda_2$ and a corresponding numerical approximate solution $\hat y \in \tau^{(K)}\Ell$ of Equation \eqref{e:eq_y} such that a pair of eigenvalues $\mu$ and $\bar \mu$ crosses the imaginary axes. Let $v$ be the  eigenvector associated to $\mu$. We set
$$
\hat z_{jk} =
\begin{cases}
v_k \qquad &\text{if } j = 1,|k|\leq K,\\
\bar v_{-k} \qquad &\text{if } j = -1,|k|\leq K,\\
0 &\text{otherwise}.
\end{cases}
$$
We also set $\hat a = 0$ as a first approximation, because we assume to be very close to a Hopf bifurcation, 
%From bifurcation theory, we can set
and we set $\hat \lambda_1$ to $|\operatorname{Im}(\mu)|^{-1}$.
This construction forms a first numerical approximation for $\hat x$. Applying Newton's method allows us to increase the accuracy of our initial approximation.
In Figure \ref{f:solution} both the stationary solution $\hat{y}$ at $\gamma\approx\gamma^*$ close to the Hopf bifurcation and the rescaled time dependent perturbation $\hat{z}$ are depicted.

Once this approximation has been constructed, the predictor-corrector algorithm, as presented for example in \cite{breden-vanicat} and \cite{QJBcontinuation}, allows us to numerically follow the solution branch. 
Then, with the method presented in this article, we rigorously validate each segment and follow the solution branch. The validated segment where   
the sign of $a$ is proven to change is where the Hopf bifurcation happens, based on 
the arguments in Remarks~\ref{r:is_Hopf} and~\ref{r:cont_eq}.


The \textsc{matlab} script \texttt{script\_HopfKS.m}, which can be found at~\cite{code}, performs the necessary computation to conclude that we have validated the existence of a Hopf bifurcation in the Kuramoto-Sivashinsky  equation from the stationary solution depicted in Figure \ref{f:solution} at parameter value $\lambda_2^* = \gamma^* =0.298776358114 +[-r,r]$ with the validation radius $r = 8.63\cdot 10^{-11}$. For the validation we used 20 temporal modes and 30 spatial modes: $K = (20,30)$. The weights used for the $\ELL$ and $\Ell$ space are $\nu = (1.1, 1.1)$. The segment has been followed from $a = -10^{-8}<0$ to $a = 5.3898\cdot 10^{-4}>0$. 
%always smaller than $1.6\cdot 10^{-10}$. 
With a step size of  $10^{-6}$, this validation required 539 steps and reached $\lambda_2 = 0.29877636757+[-r,r]$, with $r=1.6\cdot 10^{-10}$, which is at least $8 \cdot 10^{-9}$ above the bifurcation value $\lambda_2^*$.




%</conclusion>

==> correctm.tex <==
% This file defines a few macros useful in team work on a paper or a book.
% The main purpose of the macros is to faciliate having simultanously two versions
% of selected fragments of text (old and new) with appropriate comments so that
% co-authors may think before deciding which version is better.
%
% To use these macros you must put this file in the directory where you keep
% the source files and add the following two lines
%
%\include{correctm}
%\showcomments
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% at the beginnig of the main source file.
% If you want to compile the source file without any comments,
% just replace \showcomments by \hidecomments. In this case only the new versions
% will be used in the compiled text and all comments will be ommitted.
% This gives a possibility of looking at the clean text while still keeping
% the alternatives in the source file
%
% The \corrl macro
% ================
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% The main macro is \corrl and it has the following syntax
%
% \corrl comment<<old_version||new_version>>
%
% Note that <<, || and >> are obligatory even if old_version or new_version are empty texts.
% The words 'comment', 'old_version', 'new_version',
% mark the places where you put your own text, i.e. these are parameters of the macro.
% The meaning of the parameters is
%
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%     'comment'     - just a comment set in a non-standard font so that it clearly differs from
%                      the proper text
%     'old_version' - here you put the old text, which you want replaced with the new text
%     'new_version' - here you put the new text
%
% If comments are turned on by \showcomments, you will see the comment, then the old version
% clearly seperated form the new version and a margin mark. If comments are turned off, you
% will see only the new version with no comments or marks.
%
% If comment, old_version and/or new_version are longer than one line, a good idea is
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% to write this macro (as well as the following macros) as
% \corrl
%   comment
% <<
%   old_version
% ||
%   new_version
% >>
%
%
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% The \corrq macro
% ================
%
% Another possibility is that you feel some fragment should be changed but you do not know what
% should be the new version. Then use the macro
%
%  \corrq comment<<questioned_text>>
%
% With comments turned on you will see the comment followed by the clearly marked
% questioned text
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% The \corre macro
% ================
%
% Sometimes the new version is an almost obvious change, so you
% want the old version only in the source
% file (just in case ...) but not in the compiled file.
% Then use the macro
%
% \corre comment<<old_version||new_version>>
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% which in the compiled file shows only the new version and the margin mark to indicate that
% changes were made.
%
% The \corrs macro
% ================
%
% When the change is almost obvious and short, use the macro
%
% \corrs comment<<old_version||new_version>>
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% which is similar to the previous but automaticallly adds a comment
% old_version->new_version on the margin
%
% The \corrn and \corro macros
% ============================
%
% To settle matters you can use two more macros with the same syntax as \corrl
%
%  \corro - to force the old version - the new version and all comments are disregarded
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%                                      (but present in the source file)
%  \corrn - to force the new version - the old version and all comments are disregarded
%                                      (but present in the source file)
%
% This is simple in use (just replace l, q or s in the macro name by o or n) but leaves rubbish
% in the source file. If you find ourselve using plenty of this stuff one can easily write a simple PERL
% script which will automatically remove all this rubbish.
%
%
% The \corrc macro
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% ================
%
% This is to place in the source file a comment only. The syntax is
%
% \corrc comment <<>>
%
% Parameters containing whole paragraphs
% ======================================
%
% Note: the standard TeX macros cannot be called with parameters which go across paragraphs
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% (i.e. contain \par or an empty line). However, there is a special mechanism which allows for that.
% It is implemented here in the form of alternative macros \longcorrl, \longcorrq, \longcorrs and so on.
% Since TeX better recovers from errors if such macros are not present, use them only when necessary.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macro definitions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\corcommstyle{\bf\tiny}
\def\corcommstyle{\bf\small\tt}

%This macro is to be used when an alternative approach is to be displayed
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%versus the old approach

\def\corrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ {\color{red}#1\marginpar{!!}}\\$<<$OLD$<<$} \end{quote}

{\color{red} 
 #2
 }
 
 

  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
   \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
  #3
  
   \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  #3
 \fi
}

\long\def\longcorrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ {\color{red}#1\marginpar{!!}}\\$<<$OLD$<<$} \end{quote}
 
 {\color{red}

  #2
  
  }
  
  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
  
    \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
  #3
  
   \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #3
 \fi
}

\def\mlabel #1
{
  \if\visiblecomments y
     \marginpar[\flushright \bf \footnotesize #1]{\bf \footnotesize #1}
  \fi
}

\def\flabel #1
{
  \if\visiblecomments y
       \hbox{\bf\footnotesize #1}
  \fi
}


%This macro is to be used when there is some confusion
%No new text is proposed

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\def\corrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
 {\color{red}
  
  #2
  
  }
   
  \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill 
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\long\def\longcorrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill

  #2

  \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill 
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%This is just to introduce a comment

\def\corrc #1<<>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ \color{red} #1\marginpar{!!}} \end{quote}
\fi
}

%This macro is intended for some evident corrections.
%Only the new text is displayed.
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%Comment is typed on the margin.

\def\corre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\long\def\longcorre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%This macro is intended to mark corrections to short simple typos.
%Only the new text is displayed and an automatic typo change is
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%marked on the margin.

\def\corrs #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #2 $\rightarrow$ #3\\ #1}
 \else
  #3
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%The next two macros are to help settle the matters.
%Changing \corrx where x is l,q or s to \corro (\corrn)
%will result in just choosing the old (new) text.
%This is intended to provide a simple way to get rid of
%any comments, i.e. to "clean" the paper.
%Unfortunately the no longer needed versions remain
%in the source file so in the future it would be
%useful to have some preprocessor to clean also
%the source file.
%Note that since \corrq does not provide any new stuff
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%it makes sense only to change it to \corro unless some
%new text is added later on.

\def\corro #1<<#2||#3>>{
#2}

\def\corrn #1<<#2||#3>>{
#3}

\long\def\longcorro #1<<#2||#3>>{
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
#2}

\long\def\longcorrn #1<<#2||#3>>{
#3}

% This macro is to hide in official version pieces of text
% which is not available for presentation yet.

\long\def\underconstruction #1<<<#2>>>{
\if\visiblecomments y
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  \begin{quote} {\corcommstyle $<<$UNDER CONSTRUCTION - BEGIN$>>$ #1\marginpar{!!}} \end{quote}
  #2
  \begin{quote} {\corcommstyle $>>$UNDER CONSTRUCTION - END$>>$ } \end{quote}
 \else
 \fi
}



% These two macros are to tourn on/off comments
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%

\def\showcomments{
  \let\visiblecomments y
}

\def\hidecomments{
  \let\visiblecomments n
}


%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%



==> finite.tex <==
%!TEX root = HopfKS.tex

Let $K = (M,N)$ be a choice of number of modes for $\ELL$. Let $H: X\rightarrow X$ be defined as in \eqref{e:HopfKS}. We want to define the restriction of $H$ to $\tau^{(K)}X$. We then define
\begin{align}\label{e:finite_H}
\hat H :&\tau^{(K)} X &\rightarrow \tau^{(K)} X\\
&x = (\lambda_1,\lambda_2,a,y,z) &\mapsto \hat H(x),
\end{align}
with 
$$
\hat H(x) = \tau^{(K)} H(\tau^{(K)} x).
$$
This finite dimensional projection of $H$ is the numerical problem we can solve with a computer. The numerical approximation of the solution to $\hat H(x) = 0$ will be denoted by $\hat x$.

Let us remark that the derivative of $\hat H$ is also finite, that is
$$
D\hat H(x) y =\tau^{(K)} D\hat H(x) \tau^{(K)} y.
$$

\begin{remark}
In the definition of the continuation equation \eqref{e:cont_eq}, we introduced $q_i \approx \ker(DH(\hat x_i))$ for $i = 0,1$. Here we can be more specific and define
$$
q_i \approx E \ker D\hat H(\hat x_i), \qquad\text{for } i = 0,1,
$$
where the kernel is approximated numerically.
\end{remark}

Then the numerical finite dimensional problem, including the continuation equation, that we will be solving is
\begin{equation}\label{e:num_HopfKS}
H_s(\lambda_1,\lambda_2, a, y,z) = \begin{pmatrix}
\langle x, q_s\rangle + c_s\\
\langle \hat z, z\rangle -1\\
\langle\imag K   y, \hat y\rangle \\
\langle\imag K  z, 2\hat y+\hat a \hat z\rangle \\
\langle\imag J  \hat z,z\rangle \\
-\lambda_2  K^4 y +  K^2 y + 2 \imag K\Pi_K (y * y)\\
-\imag J z  +\lambda_1\lambda_2  K^4 z - \lambda_1 K^2 z + 2 \lambda_1\imag K \Pi_K(2y * z+az*z  )\\
\end{pmatrix} = 0.
\end{equation}

\begin{remark}
Let us remark that the last two equations are trivially satisfied for $k = 0 $ and $(j,k) = (0,0)$. Therefore, we will not consider the trivial equations in the computations, and we will replace them by two of the scalar equations. With this approach, the Jacobian of $H_s(x)$ will square and not singular. With this change, the dimensions requested by \eqref{e:finite_H} are satisfied. 

For sake of presentation, we will not remind the reader of this change in the ordering of the equations.
\end{remark}

==> intro_PDE.tex <==


%<*Intro>


The goal of this paper is to give a proof of a Hopf bifurcation found numerically in the Kuramoto-Sivashinsky partial differential equation (PDE) in one spatial dimension with $2\pi$-periodic boundary conditions in space:
\begin{equation}\label{e:KuramotoSivashinsky}
\begin{cases}
\partial _t u = - \partial_x^4 u - \gamma \partial^2_x u + \partial_x(u^2),\\
u(t,x) = u(t, x+2\pi).
\end{cases}
\end{equation}
Here $\gamma>0$ acts as the bifurcation parameter.
The appealing qualities of the PDE~\eqref{e:KuramotoSivashinsky} are its relative simplicity and the presence of a low order nonlinear term. Despite its simplicity, it exhibits complex dynamics, and it serves as a model for weak turbulence in laminar flows and more generally as a paradigm for studying spatiotemporal chaos. We refer to \cite{kuramoto}, \cite{sivashinsky} and \cite{sivashinsky2} for more background material on the Kuramoto-Sivashinsky equation.

In this paper we prove the existence of a Hopf bifurcation from a nonhomogeneous stationary solution to \eqref{e:KuramotoSivashinsky}  by \textit{a posteriori} validation of numerical computations. 
The Kuramoto–Sivashinsky equation has been well studied from the perspective of validated numerics. Early results include \cite{mischaikow_piotr}, where stationary solutions of \eqref{e:KuramotoSivashinsky} are found and validated. In \cite{wilczak} rigorous numerics is used to prove the existence of complicated, chaotic trajectories in the ordinary differential equation (ODE) describing steady states of the Kuramoto–Sivashinsky equation. Much more recently, by a powerful combination of a rigorous integrator for parabolic PDEs and topological arguments, the existence of an invariant set with chaotic dynamics was proven~\cite{danielpiotrchaosKS} for the semiflow induced by the PDE~\eqref{e:KuramotoSivashinsky}. 
Furthermore, the bifurcation diagram of stationary solutions of the Kuramoto-Sivashinsky equation and their stability was studied in \cite{koch_arioli}, see also \cite{piotrKS} for the pitchfork bifurcation problem. We refer to \cite{other_koch_arioli}, \cite{other_piotr}, \cite{jordi} and \cite{JP} for validation of periodic orbits in Kuramoto–Sivashinsky. Here we complement these results by an analysis of the Hopf bifurcation problem. Indeed, the periodic solutions proven in \cite{other_koch_arioli,jordi, JP,other_piotr} bifurcate from an inhomogenenous stationary state, but a mathematically rigorous analysis of this Hopf bifurcation problem has not previously been undertaken.

To tackle this, we generalize our previous desingularization work on (Hopf) bifurcations in ODEs \cite{BLQ} to the PDE setting. The main strength of this approach is that validating the existence of a Hopf bifurcation and the branch of time-periodic solutions emanating from it, is reformulated as a regular branch following problem.
The crucial advantage is that the solution branch of periodic orbits does not become singular at the bifurcation point, hence continuation can be carried out using rigorous computer-assisted pseudo-arclength continuation techniques.
There is then a straightforward correspondence between solution of the desingularized system on the one hand and those of the original system on the other.
This ``blow-up'' technique complements the approaches to computer-assisted bifurcation analysis introduced in \cite{koch_arioli} and \cite{piotrKS}. 
While we focus on Hopf bifurcations in this paper, our technique is well-suited to study more general symmetry breaking bifurcations from nonhomogeneous stationary states.

To outline the desingularization approach, it is convenient to change variables.
We consider a time $L$-periodic ($L$ being unknown for the moment), space $2\pi$-periodic solution $u(t,x)$ to \eqref{e:KuramotoSivashinsky}. We apply a time rescaling $\tau = \frac{2\pi t}{L}$ such that $ u (\tau, x)$ is time $2\pi$-periodic. The rescaled equation is written as
\begin{equation}\label{e:KuramotoSivashinskyrescaled}
\begin{cases}
\partial _\tau u = - \lambda_1\partial_x^4 u - \lambda_1\lambda_2 \partial^2_x u + \lambda_1\partial_x(u^2), \\
 u(\tau,x) = u(\tau, x+2\pi),
\end{cases}
\end{equation}
with $\lambda_1 = \frac{L}{2 \pi}$ and $\lambda_2 = \gamma$. 

If a time-dependent solution $ u(\tau,x)$  is close enough to the Hopf bifurcation, it is natural to rewrite $ u$ as the sum of a stationary solution $y(x)$ to \eqref{e:KuramotoSivashinskyrescaled} and a time-dependent perturbation $az(\tau, x)$, where $z$ is of order 1 and $a\in\mathbb{R}$ is the (small) amplitude of the perturbation. The precise formulation can be found in Section~\ref{ss:Hopf}. Following this rewriting, we  validate a branch of solutions $(\lambda_1, \lambda_2, a, y, z)$. If the amplitude $a$ changes sign along this branch, then at $a=0$ a Hopf bifurcation occurs: the periodic solutions for $a\neq 0$ bifurcate from the stationary state $y$ at $a = 0$. 

 % One could do the additional analysis without too much we coul nor do
 % \blue{I am not sure of the next paragraph: aren't we checking that $a'\neq 0$, therefore proving that the bifurcation is non-degenerate?}
 % We remark here that the Hopf bifurcation thus proven might be degenerate, since we do not check the normal form in the neighborhood of the bifurcation nor do we study the behavior of the eigenvalues of the problem. The non-degeneracy could be proven by applying the reformulation of a Hopf bifurcation into a saddle node bifurcation, as already introduced in \cite{BLQ} for ODEs and proving the existence of a saddle node in the new system. We 


%PUT THE TWO PICTURES INTO ONE.

\begin{figure}
\centerline{\hspace*{-10mm}\includegraphics[width = 0.5\textwidth]{y_new}\includegraphics[width = 0.5\textwidth]{z_sol_new}}
\caption{On the left: validated $2\pi$-periodic stationary solution $y(x)$ near the Hopf bifurcation point   .
On the right: rescaled time and space periodic profile $z(\tau,x)$ near the Hopf bifurcation.}
\label{f:solution}
\end{figure}

The validated solution close to the bifurcation is presented in Figure \ref{f:solution}, where the stationary component $y(x)$ of the solution is presented on the left and the perturbation profile $z(\tau,x)$ 
generated by the Hopf bifurcation is plotted on the right. The full solution of \eqref{e:KuramotoSivashinsky} is the sum of the stationary component and the perturbation multiplied by the amplitude $a$, which tends to zero at the bifurcation point. Thanks the the validated numerics presented in this paper, we can prove that the Kuramoto-Sivashinsky equation \eqref{e:KuramotoSivashinsky} undergoes a Hopf bifurcation at the parameter value $\lambda_2^* = \gamma^* =0.298776358114 +[-r,r]$ with validation radius $r = 8.63\cdot 10^{-11}$. 


By adding a continuation condition, we can prove that $a'\neq 0$, where the derivative is taken with respect a ``parametrization'' variable of the solution branch. This guarantees the ``non-degeneracy'' of the Hopf bifurcation in the sense that we prove a branch of non-constant periodic orbits which converge to the equilibrium state. 
In this way we avoid the need for a center manifold analysis. Furthermore, for this result we do not need to check that the conjugate eigenvalue pair, which we find at $a=0$ to lie on the imaginary axis, crosses from one side of the imaginary axis to the other side (when following the branch of stationary solution in $\gamma$). Such an analysis requires an additional computer-assisted proof, which would not be too difficult, but we did not pursue it in this paper. 
Finally, we remark that in order to establish sub- or supercriticality of the bifurcation, one could determine the sign of $a''$. In the ODE setting, this analysis has been performed in great generality in~\cite{BLQ}, and we are confident that such an approach would work in the PDE setting as well. Since working out the details is somewhat tedious and the current paper is already quite heavy on technical detail, we decided not to include it here.




% \begin{figure}
% \begin{center}
% \includegraphics[width = 0.4\textwidth]{y_sol_at_Hopf}
% \caption{Validated $2\pi$-periodic stationary solution at the Hopf bifurcation point.
% }\label{f:y}
% \end{center}
% \end{figure}
%
%
% \begin{figure}
% \begin{center}
% \includegraphics[width = 0.7\textwidth,trim={2cm 7cm 2cm 8cm},clip]{z_sol_at_Hopf.pdf}
% \caption{Rescaled time and space periodic profile $z$ near the Hopf bifurcation.
% }\label{f:z}
% \end{center}
% \end{figure}
% \blue{ update picture code to make is lighter and prettier}

% \red{end figure section}


The details of the result presented graphically in Figure~\ref{f:solution} are discussed in Section \ref{s:conclusion}. The main challenge in transforming the ODE methods in \cite{BLQ} to the PDE setting of the current paper are two-fold. First, the two-dimensional Fourier series lead to diagonally dominant operators, whose diagonal depends on the \emph{a priori} unknown time period $\lambda_1$.
This requires additional estimates to perform the tail (truncation) estimates. Furthermore, the nonlinearity includes a derivative, which can be controlled because it is lower order than the bi-Laplacian, but again this requires additional bounds. Both of these are discussed in Section~\ref{s:tail}.
We stress 
 that lifting the techniques from ODEs to PDEs is \emph{not} difficult from a technical point of view. One may find this disappointing, but we view it as the pivotal strength of the approach.
%  the relative ``straight''
%\blue{is this a reasonable sentence or should it be avoided? $->$}
%\red{In fact I reformulated it to to stress it even more. Perhaps this is a risk, but one I am happy to take.}
% As a general statement, it is remarkable how congruous the ODE and PDE problems are in the chosen functional analytic framework on Fourier space.
Indeed, the blow up approach presented is extremely general in its simplicity. % The extension of the method to a broader class of PDEs is relatively straightforward, although beyond the scope of this article. In addition,
It seems probable that the bounds developed in this paper can be applied with minor modifications to many other parabolic PDEs with periodic (or Neuman) boundary conditions. 
%\blue{ how can you say: this is the very close nex step in this project?}


The outline of the paper is as follows. In Section~\ref{s:problem} we introduce the functional analytic setup, which  
 is analogous to that of \cite{JP} and~\cite{jordi}, employing Fourier series and a convenient choice of the norm in Fourier space. The quantitative contraction theorem of Newton-Kantorovich type, which underlies the computer-assisted proof, is presented in Section~\ref{s:radii_pol}.
Sections~\ref{s:linop_in_ELL} and~\ref{s:A} are devoted to introducing and bounding the relevant projections and other linear operators. The necessary results for analyzing the tails of the Fourier modes are collected in Section~\ref{s:tail}. In Section~\ref{s:singlebounds} the ``Newton-Kantorovich'' bounds for single periodic orbits are derived. Subsequently, these are generalized to bounds for the continuation case in Section~\ref{s:cont_bound}. Finally, in Section~\ref{s:conclusion} we collect all ingredients to prove the existence result discussed above.


%</Intro>


==> linop_in_ELL.tex <==
%<*linop>

\subsection{Operators on $X$}
For simplicity, we introduce the notation $X = X_1\times X_2\times X_3$, where $X_1 = \mathbb{C}^3,\, X_2 = \Ell,\, X_3 = \ELL$. Let $B\in B(X,X)$,
\begin{align*}
B:X\qquad&\rightarrow X\\
x = (a,b,c)& \mapsto Bx = (a',b',c'),
\end{align*}
which we write as
\begin{align}\label{e:notation_Xop}
\begin{pmatrix}
a'\\b'\\c'
\end{pmatrix} = 
\begin{pmatrix}
B_{11} & B_{12} & B_{13}\\
 B_{21} & B_{22} & B_{23}\\
 B_{31} & B_{32} & B_{33}
\end{pmatrix}\begin{pmatrix}
a\\b\\c
\end{pmatrix}
\end{align}
with
$$
B_{ij}\in B(X_i,X_j).
$$
We denote by $\|\cdot\|_{ij}$ the operator norm induced by the norms on $X_i$ and $X_j$. In particular, all the operator norms here introduced have a simple explicit form or bound:
\begin{align}\label{e:sub_norm}
&\|B_{11} \|_{11} = \max_{n = 1,2,3} \sum_{m = 1,2,3}  |B_{nm}|,
\nonumber
\\\nonumber&\|B_{12} \|_{12} = \max_{n = 1,2,3} \sup_{k\in\mathbb{Z}} \nu^{-|k|} |B_{nk}|,
\\\nonumber&\|B_{13} \|_{13} = \max_{n = 1,2,3} \sup_{(j,k)\in\mathbb{Z}^2} \nu^{-|k|-|j|} |B_{nk}|,
\\\nonumber&\|B_{21} \|_{21} \leq \sum_{m = 1,2,3} \sum_{k\in\mathbb{Z}}  \nu^{|k|} |B_{km}|,
\\&\|B_{22} \|_{22} =\sup_{k_1\in\mathbb{Z}}\nu_2^{-|k_1|}\sum_{k\in\mathbb{Z}}\nu_2^{|k|}|B_{kk_1}|
\\\nonumber&\|B_{31} \|_{31} \leq \sum_{m = 1,2,3} \sum_{(j,k)\in\mathbb{Z}^2}\nu^{|k|+|j|} |B_{jkm}|
\\\nonumber&\|B_{32} \|_{32} = \sup_{k_1\in\mathbb{Z}}\nu_2^{-|k_1|}\sum_{j,k\in\mathbb{Z}}\nu_1^{|j|}\nu_2^{|k|}|B_{jkk_1}|
\\\nonumber&\|B_{33} \|_{33} =\sup_{j_1,k_1\in\mathbb{Z}}\nu_1^{-|j_1|}\nu_2^{-|k_1|}\sum_{j,k\in\mathbb{Z}}\nu_1^{|j|}\nu_2^{|k|}|B_{jj_1kk_1}|.
\end{align}
The norm $\|\cdot\|_{23}$ is not presented because it is never used in this paper.


On $B(X,X')$, we introduce the component norm
$$
\|B\|_c = \begin{pmatrix}
\|B_{11}\|_{11} & \|B_{12}\|_{12} & \|B_{13}\|_{13}\\
 \|B_{21}\|_{21} & \|B_{22}\|_{22} &\| B_{23}\|_{23}\\
\| B_{31}\|_{31} & \|B_{32}\|_{32} & \|B_{33}\|_{33}
\end{pmatrix}\in\mathbb{R}^{3\times 3}.
$$
By the definition of operator norm on the space $X$, we have
\begin{equation}\label{e:split_op_norm}
\|B\| \leq \max_{j = 1,\dots, 3} \sum_{i = 1,\dots,3} \| B_{ij}\|_{ij}.
\end{equation}



\subsection{Convolution operators on $\Ell$ and $\ELL$}

For $u = (u_k)_{k\in\mathbb{Z}} \in\Ell$, we 
%Let us consider $u$, an element of $\Ell$. We  
introduce the convolution operator  as the operator $C^{\Ell}:\Ell\rightarrow B(\Ell,\Ell)$ that satisfies 
\begin{equation}%\label{e:conv_op}
C^{\Ell}(u) w = u * w \qquad\text{for all }u,w\in\Ell.
\end{equation}
By the definition of convolution, 
%it follows that, for $u = (u_k)_{k\in\mathbb{Z}} \in\Ell$, the 
its matrix representation 
%of $C^{\Ell}$ 
is
$$
{C^{\Ell}(u)}_{k_1k_2}  =  {u}_{k_1-k_2}.
$$
It follows from the Banach algebra property that 
\begin{equation}\label{e:conv_op_norm1}
\| C^{\Ell}(u)\|_{B(\Ell, \Ell)} = \|u\|_{\Ell}.
\end{equation}
 
Following the same structure in $\ELL$, we  introduce the convolution operator $C^{\ELL}:\ELL\rightarrow B(\ELL,\ELL)$ such that
\begin{equation}\label{e:conv_op}
C^{\ELL}(u) w = u * w \qquad\text{for all }u,w\in\ELL.
\end{equation}
% By the definition of convolution, the matrix representation of $C^{\ELL}(u)$ is
We now have 
$
{C^{\ELL}(u)}_{j_1j_2k_1k_2}  =  {u}_{j_1-j_2k_1-k_2},
$
and 
%it follows from the Banach algebra property that 
\begin{equation}\label{e:conv_op_norm}
\| C^{\ELL}(u)\|_{B(\ELL, \ELL)} = \|u\|_{\ELL}.
\end{equation}




\subsection{Finite dimensional projection}

In order to study a finite dimensional subset of $X$, we define for any $K= (M,N)\in\mathbb{N}^2$ the finite set of indices smaller than $K$ as
%We will also be using the notation
\begin{equation}\label{e:finite_index}
\F = \F[(M,N)] = \{(j,k)\in  \mathbb{Z}^2\,|\,|j|\leq M, |k|\leq N \} .
\end{equation}
The projection on the first $K=(M,N)\in\mathbb{N}^2$ modes is defined as
\begin{align}
\Pi^{(K)} :\quad X=\mathbb{C}^3\times \ell^1_{\nu_2}\times \ELL &\rightarrow X\\ \nonumber
x= (a,b,c)& \mapsto \Pi^{(K)} x = (a,\Pi^{(K)}_1 b, \Pi^{(K)}_2 c)
\end{align}
with 
\begin{align}
(\Pi_1^{(K)} b)_k =\begin{cases} b_k  \quad &\text{if } |k|\leq N,\\0 \quad &\text{if } |k|>N,\end{cases}
\end{align}
and 
\begin{align}
(\Pi_2 ^{(K)}c)_{jk} =\begin{cases}  
c_{jk}  \quad &\text{if } (j,k)\in \F[(M,N)] ,\\0 \quad &\text{if } (j,k)\notin \F[(M,N)].\end{cases}
\end{align}
If $x = \Pi^{(K)}x\in X$, we say that $x$ has at most $K$ non-zero modes, and similarly for $b = \Pi ^{(K)}_1 b\in\Ell$ and $c = \Pi ^{(K)}_2 c\in \ELL$. The complementary projection on the infinite tail is given by
\begin{equation}\label{e:tail}
\Infty x  = x - \Proj x,
\end{equation}
where the notation is meant to indicate the projection from the $(K+1)$-th mode onwards. There is a natural correspondence between $\Pi_1^{(K)}\ell^1_{\nu_2}$ and $\mathbb{C}^{2N+1}$, which we denote by the truncation operator
\begin{align}
\tau^{(K)}_1:\Ell&\rightarrow \mathbb{C}^{2N+1},\\
b&\mapsto (b_k)_{k=-N,\dots, N},
\end{align}
 as well as between  $\Pi_2^{(K)}\ELL$ and $\mathbb{C}^{(2M+1)\times(2N+1)}$, which we indicate by
\begin{align}
\tau^{(K)}_2:\ELL&\rightarrow \mathbb{C}^{(2M+1)\times(2N+1)},\\
c&\mapsto (c_{jk})_{(j,k)\in \F}.
\end{align}
We introduce the notation for truncation in $X$ as
\begin{align}
\tau^{(K)} :\quad\quad\quad\quad X &\rightarrow \mathbb{C}^3\times \mathbb{C}^{2N+1}\times\mathbb{C}^{(2M+1)\times(2N+1)}\\
x= (a,b,c)& \mapsto \tau^{(K)} x = (a,\tau^{(K)}_1 b, \tau^{(K)}_2 c).
\end{align}
Its corresponding inverse embedding is denoted by
$$E: \mathbb{C}^3\times \mathbb{C}^{2N+1}\times\mathbb{C}^{(2M+1)\times(2N+1)} \rightarrow \Pi^{(K)}X.$$


\begin{definition}
$A\in\mathcal{B}(X,X)$ is a \emph{finite linear operator of center dimensions $K_1$ and $K_2$} if
$$
Ax = \Pi^{(K_1)}(A\Pi^{(K_2)}x),\qquad\text{for all } x\in X.
$$
If $K_1 = K_2=K$, we say that $A$ has center dimension $K$. 
\end{definition}

\begin{remark}\label{r:dim_fin_op}
A finite linear operator $A \in B(X,X)$ of center dimensions $K_1 = (M_1,N_1)$ and $K_2=(M_2,N_2)$ can be represented by a complex matrix of dimension $(3+(2N_2+1)+(2M_2+1)(2N_2+1))\times (3+(2N_1+1)+(2M_1+1)(2N_1+1))$.
\end{remark}

A class of operators we will be working with extensively is the class of eventually diagonal operators in $X$. It is an extention of the definition provided in \cite{JP} for eventually diagonal operators in $\ell^1_\nu$.

\begin{definition} \label{d:eventually_diag}
Let 
$
A : X \rightarrow X
$ be a linear operator. $A$ is eventually diagonal of center dimension $K$ if it can be decomposed into $A^F$ and $A^I$ such that
$$
A x =  A^F x + A^I \Infty y
$$ 
with $A^I$ a diagonal operator and $A^F$ a finite linear operator of center dimension~$K$.  The same definition applies for $A:\ell^1_\nu\rightarrow\ell^1_\nu$ and $A:\ELL\rightarrow\ELL$.
\end{definition}


\begin{lemma}\label{l:eventual_diag}
If $A$ is eventually diagonal,
$$
\| A_{ij}\|_{ij} \leq\max\{ \|A^F_{ij}\|_{ij} , \| A^I_{ij}\|_{ij} \},
\qquad \text{for } i,j=1,2,3.
$$
%for $i,j=1,2,3$.
\end{lemma}
\begin{proof}
Let $A= A^I+A^F$ be an eventually diagonal operator of center dimension $K = (M,N)$. 
%Let's concentrate on computing all the component wise norms.
For $i\neq j$, $A^I_{ij}=0$, and $A^I_{11} = 0$, hence in these cases $\|A_{ij}\| = \|A^F_{ij}\|$. We are left to compute $\|A_{22}\|_{22}$ and $\|A_{33}\|_{33}$. By the definition of the norms in \eqref{e:sub_norm}, we have
\begin{align*}
\|A_{22}\|_{22} &= \sup_{k_2\in\mathbb{Z}} \nu_2^{-|k_2|}\sum_{k_1\in\mathbb{Z}}\nu_2^{|k_1|} |(A_{22})_{k_1k_2} \\
&= \max \{ \sup_{|k_2|\leq N} \nu_2^{-|k_2|}\sum_{k_1\in\mathbb{Z}}\nu_2^{|k_1|} |(A_{22})_{k_1k_2}| ,\\ &\hspace{2cm} \sup_{|k_2|>N} \nu_2^{-|k_2|}\sum_{k_1\in\mathbb{Z}}\nu_2^{|k_1|} |(A_{22})_{k_1k_2}| \}\\
& = \max \{ \sup_{|k_2|\leq N} \nu_2^{-|k_2|}\sum_{k_1\in\mathbb{Z}}\nu_2^{|k_1|} |(A^F_{22})_{k_1k_2} , \sup_{|k_2|>N} |(A^I_{22})_{k_1k_1} |\}\\
& = \max \{ \|A^F_{22}\|_{22} , \|A^I_{22}\|_{22}\}.
\end{align*}
The same approach can be applied to $A_{33}$, thus concluding the proof.
\end{proof}
\begin{remark}
The product of two eventually diagonal operators of center dimensions $K_1$ and $K_2$, respectively, is an eventually diagonal operator of center dimension
$$
K = \max\{K_1,K_2\}.
$$
\end{remark}

The operator $A$ introduced in Section \ref{s:radii_pol} will be constructed to be an eventually diagonal operator. We therefore want to study this type of operators a little more in depth.

\begin{remark}\label{l:sizeAy}
Let $x\in X$ such that $x = \Pi^{(K')}x$,  and let $A$ be an eventually diagonal operator of center dimension $K$, then 
$$
Ax = \Pi^{(\tilde K)}(Ax),
$$
with
$$
\tilde K = \max(K,K').
$$
\end{remark}


Another case in which it is easy to compute the  number of non-zero modes is when we are considering convolutions.

\begin{lemma}\label{l:conv_size}
Let  $x = \Pi^{(K_1)}_2x  $ and $ v= \Pi_2^{(K_2)}v$ then 
$$
x*v = \Pi^{(K_1+K_2)}_2 (x*v) .
$$
The same holds in $\Ell$.
\end{lemma}

We also introduce the definition of a $K$-diagonal operator, where $K$ can be thought of as a band width.

\begin{definition}\label{def:K_diag}
$B:X\rightarrow X$ is called a $K$-diagonal operator on $X$ if 
$$
By = \Pi^{(K+K')}(By)
$$
for all $y\in X$ such that $y = \Proj[ (K')]y$.
And similarly for $B:\ELL\rightarrow \ELL$ and $B:\ell^1_{\nu_2}\rightarrow \ell^1_{\nu_2}$.
% Similarly, if $B:\ELL\rightarrow \ELL$ and
% $
% By = \Pi^{(K+K')}_2(By)
% $ for any $y\in \ELL$ with $K'$ non-zero modes, then $B$ is a $K$-diagonal operator in $\ELL$, and the same definition can be applied to operators on $\ell^1_{\nu_2}$.
\end{definition}

\begin{remark}
%It is obvious by the definition that d
Diagonal operators are 1-diagonal operators. Furthermore, by Lemma \ref{l:conv_size}, the convolution operators associated to $y\in \ell^1_{\nu_2}$ and $z\in \ELL$ with $K$ non-zero modes are $K$-diagonal.
\end{remark}

\begin{lemma}
 $B$ is a $K$-diagonal operator in $\ELL$ if and only if its matrix representation $B$ is such that $B_{jj_1kk_1} = 0$ if $(j - j_1, k-k_1) \notin \F$.
A similar statement holds in $\Ell$.
\end{lemma}

\begin{lemma}
Let $K = (M,N) \in \mathbb{N}^2$, and let $B:X\rightarrow X$ be a $K$-diagonal linear operator. Then $B_{22}:\Ell\rightarrow \Ell$ is a $K$-diagonal linear operator and so is $B_{33}:\ELL\rightarrow \ELL$. For $B_{32}:\Ell \rightarrow \ELL$, its matrix representation $B_{32}$ is such that $(B_{32})_{j k k _1}  = 0 $ if $|k - k_1|>N$.
\end{lemma}
%We do not discuss $B_{23}$ because it vanishes for all the operators treated in this paper.% it holds $B_{23}=0$.

\begin{theorem}\label{t:size_op_prod}
Let $A:X\rightarrow X$ be a finite dimensional operator of center dimension $K_1=(M_1,N_1)$ and $K_2 = (M_2,N_2)$. Let $B:X\rightarrow X$ be a $\tilde K$-diagonal operator. Then the operator product $AB$ is a finite dimensional operator of center dimension $K_1$ and $K_2+\tilde K$.


\end{theorem}
\begin{proof}
The proof will be carried out for $A' = A_{22}$ and $B' = B_{22}$, but its extension to the whole of $X$ follows the same reasoning.

By definition of the operator product, it holds that  $$(A'B')_{k_1k_2} = \sum_{k_3\in\mathbb{Z}} A'_{k_1k_3} B'_{k_3 k_2}.$$ The assumptions imply that $A'_{k_1k_3} = 0$ if $k_1 > N_1$ or $k_3>N_1$. Furthermore, $B'_{k_3 k_2} = 0$ if $|k_3-k_2|>\tilde N$. Hence, we can rewrite
$$
(A'B')_{k_1k_2} = \sum_{k_3\in I_{k_2}} A'_{k_1k_3} B'_{k_3 k_2},
$$
with 
$$
I_{k_2} = \{ k_2 - \tilde N, \dots, k_2 +\tilde N\} \cap \{ -N_2, \dots, N_2\}.
$$
The set $I_{k_2}$ is non-empty only if $|k_2|\leq N_2+\tilde N$. This concludes the proof.
\end{proof}


\begin{corollary}\label{l:finite_norm}
Under the hypothesis of Theorem \ref{t:size_op_prod}, 
we have
$$
AB = \Pi^{(K_1)} A \Pi^{(K_2)}  B = \Pi^{(K_1)} A \Pi^{(K_2)} B \Pi^{(K_2+\tilde K)}.
$$
Hence, (a bound on) the operator norm $\|AB\|$ is explicitely computable.
% , since it depends on just a finite number of indices of the matrix representation of $B$, namely on $\Pi^{(K_2)} B \Pi^{(K_2+\tilde K)}$.
\end{corollary}

%</linop>



==> operator_A.tex <==
%<*operator-A>

In this Section, we construct the operator $A_s$ needed for the application of the radii polynomial approach to the Kuramoto-Sivashinsky PDE given by \eqref{e:HopfKS_cont}. We consider the segment
$$
\hat x_s  = E\hat x_0 + s(E\hat x_1 - E\hat x_0),
$$
where $\hat x_0, \hat x_1 \in \tau^{(K)} \mathcal{S}(X)$ are the two  numerical approximate solutions of \eqref{e:HopfKS_cont} already introduced at the end of Section \ref{s:problem}.

The radii polynomial approach to the validation of a branch relies strongly on finding  a reasonably good approximation $A_s$ of the inverse of $DH_s(\hat x_s)$. To construct $A_s$, we will introduce the linear operator $A^\dagger_s$, an approximation of $DH_s(\hat x _s)$. First, let us compute explicitly
\begin{multline}
DH_s( x) = \\\tilde \Pi
\begin{pmatrix}
D_{(\lambda_1,\lambda_2,a)}\begin{pmatrix}\Es( x)\\ G(x)\end{pmatrix}  & D_{y}\begin{pmatrix}\Es( x)\\ G(x)\end{pmatrix} & D_{z}\begin{pmatrix}\Es( x)\\ G(x)\end{pmatrix}\\
D_{(\lambda_1,\lambda_2,a)}F_1(x)& 
\lambda_2\K^4-\K^2- 2\imag \K C^{\Ell}( y) 
& 0\\
D_{(\lambda_1,\lambda_2,a)}F_2(x)
& -2\lambda_1\imag \K C^{\ELL} (z) E_\ell &\begin{smallmatrix}
\imag \J +\lambda_1\lambda_2 \K^4 - \lambda_1\K^2 \\-
2\lambda_1\imag \K C^{\ELL}( E_\ell y+a z) 
\end{smallmatrix}
\end{pmatrix}.
\end{multline}
with
\begin{align*}
D_{(\lambda_1,\lambda_2,a)}F_1(x)&=\begin{pmatrix}0 & \K^4y & 0 \end{pmatrix},\\
D_{(\lambda_1,\lambda_2,a)}F_2(x)&=\begin{pmatrix}
\begin{smallmatrix}
(\lambda_2\K^4-\K^2)z\\ -\imag \K
(2z*E_\ell y+a (z*z))
\end{smallmatrix} & \lambda_1 \K^4z & 
-\lambda_1\imag \K (z*z) 
\end{pmatrix},
\end{align*}

We define 
$$
\hat H_s(x) \bydef \tau^{(K)} H_s(\tau^{(K)} x),
$$
which can be interpreted as a map from $\mathbb{C}^{3+(2N+1)+(2N+1)(2M+1)}$ to itself, and we have
\begin{equation}
D \hat H_s( x) = \tau^{(K)} DH_s(\tau^{(K)} x)\tau^{(K)} ,
\end{equation}
which can be represented by a complex square matrix of dimensions $(3+(2N+1)+(2N+1)(2M+1))$.

We construct  the dependence of $A^\dagger_s$ on $s$ to be linear:
$$
A^\dagger_s = A^\dagger_0 + s(A^\dagger_1-A^\dagger_0),
$$
where we define $A^\dagger_\s$  as
$$
A^\dagger_\s = E D\hat H_\s (\hat x_\s)+ A^{\dagger I}_\s, \qquad \text{for } \s = 0,1,
$$
with $A^{\dagger I}_\s$  the tail operator

$$
A^{\dagger I}_\s =\begin{pmatrix}
0&0&0\\
0&  
\hat \lambda_{2\s}\K^4-\K^2& 0\\
0 
 & 0&
\imag\J + \hat \lambda_{1\s }\hat \lambda_{2\s} \K^4 -  \hat \lambda_{1\s}\K^2 
\end{pmatrix}\Infty.
$$

For the approximate inverse $A_s$ of $A^\dagger_s$, we set
$$
A_s = A_0 + s(A_1 - A_0),
$$
and 
$$
A_\s = A_\s^F + A_\s^I,\qquad \text{for } \s= 0,1,
$$
with
$$
A^F_\s = EQ_s\tau^{(K)}, \qquad \text{for } \s = 0,1,
$$
where $Q_s$ is an approximate numerical inverse of the matrix representation of $D\hat H_\s(\tau^{(K)}x_\s)$, a complex square matrix of dimension $(3+(2N+1)+(2N+1)(2M+1))$. The diagonal operators are defined as
\begin{equation}\label{e:Ai}
A^I_\s =
\begin{pmatrix}
0&0&0\\
0& 
 A^I_{\s1} & 0\\
0  & 0 &
A^I_{\s2}
\end{pmatrix}\Infty,
\end{equation}
with
$$
A^I_{\s1} = (\hat \lambda_{2\s}\K^4-\K^2) ^{-1} 
$$
and
$$
A^I_{\s2} = (\imag \J + \hat \lambda_{1\s} \hat \lambda_{2\s} \K^4 -  \hat \lambda_{1\s}\K^2 )^{-1} ,
$$
where the inverse here is interpreted elementwise, that is, for $(j,k)\notin \F$,
$$
(A^I_{\s 1} y)_k = \frac{y_k}{  \hat \lambda_{2\s}k^4-k^2},
$$
and
$$
(A^I_{\s 2} z)_{jk} = \frac{z_{jk}}{\imag j + \hat \lambda_{1\s} \hat \lambda_{2\s} k^4 -  \hat \lambda_{1\s}k^2}.
$$


%\red{check the conditions on $A_s$ $->$}
In Equation \eqref{conditions_A} we stated two conditions which $A_s$ needs to satisfy. First, we require that $A_sH_s(x)\in X$ for all $x\in X$. Although $H_s(x)$ is not in $X$ due to the unboundedness of the operators $\J$ and $\K$, this is counteracted by the action of the tail of $A_s$, hence $A_sH_s(x)\in X$.%therefore the first condition on $A_s$ is satisfied.
 
The second condition is that $A_s$ is injective. This condition is proven \emph{a posteriori} by the radii polynomial approach. Indeed, if the validation succeeds, it holds that $1>Z(r)\geq \sup_{s\in[0,1]}\| I - A_sA^\dagger_s\|$, thus $A_s$ is surjective for all $s\in [0,1]$. We also know that $A_s$ is eventually diagonal for all $s$, that is $A_s = A_s^F + A_s^I$. 
We now interpret this as a block-diagonal decomposition of $A_s$.
Then, by surjectivity of $A_s$, we deduce surjectivity of $A_s^F$, and since $A^F_s$ is finite dimensional, surjectivity implies injectivity. 
%Finally 
Injectivity of $A_s^I$ follows from the nontrivially of the elements on its diagonal.
Hence $A_s$ is injective.

\begin{remark}
The elements on the diagonal are nontrivial if $\hat \lambda_{2\s} k^4-k^2 \neq 0 $ for all $|k|>N$. Thus we impose
$$
N^2>\max \{ \hat \lambda_{20}^{-1},\hat \lambda_{21}^{-1}\}.
$$
\end{remark}


%</operator-A>

==> problem.tex <==


%<*problem>

\subsection{The Kuramoto-Sivashinsky equation}\label{ss:standard}

In Section \ref{s:intro}, we rescaled the Kuramoto-Sivashinsky equation to
\begin{equation}\label{e:KS}
\partial_t v = -\lambda_1\lambda_2 \partial_{x}^4 v- \lambda_1\partial_{x}^2v + 2\lambda_1 \partial_{x}(v^2),
\end{equation}
so that we can study solutions which are $2\pi$-periodic in space and time.

To write $v$ in terms of its Fourier expansion in $t$ and $x$ we introduce the two-dimensional bi-infinite sequence $u =(u_{jk})_{j,k\in\mathbb{Z}}$, with $u_{jk}\in\mathbb{C}$, such that 
\begin{equation}\label{e:Fourier}
v(t,x) = \sum_{j,k\in\Z} u_{jk} e^{\imag (j t+k x)} .
\end{equation}
From here onwards, we will consistently use $j$ for time related indices and $k$ for space related indices.
We introduce the notation 
$$
\mathcal{F}v = u
$$
 for the two-dimensional Fourier transform, with $u$ defined above.
 
We recall some standard properties of Fourier sequences that will be used extensively in the following.
 The convolution of  two two-dimensional bi-infinite sequences $u$ and $w$  is defined by
$$
(u*w)_{jk} = \sum_{j_1+j_2=j}\sum_{k_1+k_2=k} u_{j_1k_1}w_{j_2k_2}.
$$
Furthermore it holds that
$$
u*w = \mathcal{F}(\mathcal{F}^{-1}(u)\cdot \mathcal{F}^{-1}(w)) ,
$$
where $\mathcal{F}^{-1}$ is the inverse Fourier transform and the multiplication $\cdot$ is considered pointwise in $t$ and $x$. The derivative operators satisfy
$$
\mathcal{F}(\partial_t v(t,x)) =( \imag ju_{jk} )_{j,k\in\mathbb{Z}}\quad
\text{ and }\quad
\mathcal{F}(\partial_x v(t,x)) =( \imag ku_{jk} )_{j,k\in\mathbb{Z}}.
$$
We denote the multiplication of a two-dimensional bi-infinite sequence by its index in the time or space direction by the operator $\J$ or $\K$, respectively, defined as
\begin{align}\label{e:op_J}
\J : u \mapsto  (ju_{jk})_{j,k\in\mathbb{Z}}
\end{align}
and
\begin{align}\label{e:opK}
\K:u \mapsto   (ku_{jk})_{j,k\in\mathbb{Z}}.
\end{align}
% Thus we are able to write
% $
% \mathcal{F}(\partial_t v)= \imag  \J \mathcal{F}(v)
% $ and
% $
% \mathcal{F}(\partial_x v) = \imag \K \mathcal{F}(v)
% $.
%
%
%Using the notation just introduced, we can 
We rewrite Equation \eqref{e:KS} in the space of Fourier sequences as
\begin{equation}
\imag \J u = -\lambda_1\lambda_2 \K ^4 u + \lambda_1\K^2 u +  \imag \lambda_1\K (u * u)  ,
\end{equation}
and we introduce the zero finding problem
\begin{equation}\label{e:KSF}
f(\lambda_1,\lambda_2,u) \bydef  \imag \J u  + \lambda_1\lambda_2  \K^4 u - \lambda_1 \K^2 u -  \imag\lambda_1 \K (u * u) =0 .
\end{equation} 

% \begin{remark}
% In Equation \eqref{e:KS}, the last term is
% $
% 2vv_x = (v^2)_x
% $. The first formulation would be rewritten as $2u*(\imag \K u)$ in Fourier sequences, while the second one corresponds to $\imag \K(u*u)$. They are equivalent, but the second one is chosen in this paper because it makes the notation for derivatives simpler.
% \end{remark}

\begin{remark}\label{r:f00}
Writing explicitly
$$
f_{jk}(\lambda_1,\lambda_2,u) =  \imag ju_{jk}  + \lambda_1\lambda_2  k^4 u_{jk} - \lambda_1 k^2 u_{jk} -  \lambda_1\imag k (u * u) _{jk},\qquad j,k\in\mathbb{Z},
$$
 we notice that $f_{00}(\lambda_1,\lambda_2,u) \equiv 0$.
\end{remark}
When $u$ is a solution to \eqref{e:KSF}, any shift in time or space of $u$ is also a solution. In order to lift this invariance, we  add two  phase conditions to our problem of the form
\begin{equation}\label{e:phase_cond}
\langle \imag \K \tilde u,u\rangle = 0\quad \text{and} \quad \langle \imag \J \tilde u,u\rangle = 0,
\end{equation}
where $\tilde u$ is an approximation of the solution and
$$
\langle u,w\rangle=\sum_{j,k\in\mathbb{Z}}u_{jk}w_{jk},
$$
for $u,w\in\mathbb{C}^{\mathbb{Z}^2}$. Conditions \eqref{e:phase_cond} are the Fourier sequence representations of
$$
\int_0^{2\pi} v \tilde v_xdx = 0 \quad \text{ and } \int_0^{2\pi} v \tilde v_tdt = 0,
$$
with $\tilde v$ a numerically determined approximation of the solution. These are standard conditions to fix shifts (see e.g.~\cite{QJBcontinuation}).

The full problem then becomes
\begin{equation}\label{e:full_KSF}
\begin{cases}
f_{jk}(\lambda_1,\lambda_2,u) = 0,\qquad\text{for all } (j,k)\in\mathbb{Z}^2\backslash \{(0,0)\}, \\
\langle \imag \K \tilde u,u\rangle = 0,\\
\langle \imag \J \tilde u,u\rangle = 0,
\end{cases}
\end{equation}
and one expects a one-dimensional solution branch, due to the two parameters, two scalar equations and considering Remark \ref{r:f00}.

\subsection{The functional spaces $\Ell$ and $\ELL$}

In this section, we introduce the spaces of one and two-dimensional bi-infinite sequences. Following \cite{breden-vanicat}, for one-dimensional bi-infinite sequences we introduce the norm
\begin{equation}%\label{e:normL1}
\| u\|_{\Ell} \bydef \sum_{k\in\mathbb{Z}}  \nu_2^{|k|} |u_{k}|,
\end{equation}
and the space of one-dimensional exponentially decreasing sequences as
$$
\Ell = \{ u = (u_{k})_{k\in\mathbb{Z}}, \, u_{k}\in\mathbb{C} \,|\, \| u \|_{\Ell}<\infty\}.
$$
The convolution of two sequences $y$ and $w$ in  $\ell^1_{\nu_2}$ is defined as
$$
(y*w)_k = \sum_{k_1+k_2 = k} y_{k_1} w_{k_2}.
$$

The norm and space introduced for bi-infinite sequences are very similar. For a given vector $\nu = (\nu_1,\nu_2)$, with $\nu_i\geq 1$ for $i=1,2$, we introduce the $\ELL$-norm in the space of bi-infinite sequences 
\begin{equation}\label{e:normL1}
\| u\|_{\ELL} \bydef \sum_{j,k\in\mathbb{Z}} \nu_1^{|j|} \nu_2^{|k|} |u_{jk}|,
\end{equation}
that is the two-dimensional version of the norm already used in \cite{QJBcontinuation}. It resembles closely the norm used in other papers discussing Kuramoto-Sivashinsky, such as \cite{jordi} and \cite{JP}. In particular, the $\ELL$-norm has similar properties to the $M$-norm presented in \cite{jordi}. We define the space of two-dimensional exponentially decreasing sequences as
$$
\ELL = \{ u = (u_{jk})_{j,k\in\mathbb{Z}}, \, u_{j,k}\in\mathbb{C} \,|\, \| u \|_{\ELL}<\infty\}.
$$
% It is then clear that $\ELL$ is an extension of the  $\Ell$ space for two-dimensional sequences where the exponential decrease in the first index is determined by $\nu_1$ and in the second index by $\nu_2$. 
%The presence of twodifferent indices allows for more freedom in the choice of the normed space.
%This is particularly interesting in our case, where we expect the time dependence to be simple due to the vicinity of a Hopf bifurcation, while we have no such knowledge for the space dependence.

The $\ELL$ space shares a lot of properties with the  $\ell^1_{\nu_2}$ space. First, $\ELL$ is a Banach space, and
$$
\| u*v\|_{\ELL} \leq \| u\|_{\ELL}\|v\|_{\ELL}.
$$
Furthermore, there is a trivial embedding of $\ell^1_{\nu_2}$ in $\ELL$ 
\begin{align*}
E_{\ell}:\ell^1_{\nu_2}\rightarrow&\ELL\\
 y \mapsto & E_{\ell} y: (E_{\ell} y)_{jk} = \delta_{j0} y_k,
\end{align*}
which satisfies $\|y\|_{\ell^1_{\nu_2}} = \|E_{\ell} y\|_{\ELL}$. Thanks to this embedding, we can make sense of the convolution between an element $y$  of  $\ell^1_{\nu_2}$ and an element $u$ of $\ELL$, defining it as
$$
(y*u)_{jk} \bydef (E_{\ell} y*u)_{jk} = \sum_{k_1+k_2 = k} y_{k_1} u_{jk_2}.
$$



\subsection{The Hopf bifurcation}\label{ss:Hopf}

A sequence $y\in\ell^1_{\nu_2}$ is a stationary solution of \eqref{e:KSF} if it satisfies
\begin{equation}\label{e:eq_y}
F_1(\lambda_2,y)\bydef \lambda_2 \K^4 y -  \K^2 y -  \imag \K (y * y) =0.
\end{equation}
%where the  equation is considered in $\Ell$. 
We remark that $(F_1)_0=0$ is trivially satisfied. To avoid shifts in space of the solution to \eqref{e:eq_y}, as we did for the time-dependent solution in Section \ref{ss:standard}, we add the phase condition 
\begin{equation}\label{e:pc_y}
%\langle\imag E_\ell\K  \tilde y, E_\ell y\rangle= \sum_{k\in\mathbb{Z}} \imag k \tilde y_k y_k =0,
\langle\imag \K  \tilde y,  y\rangle_\ell \bydef\langle\imag E_\ell\K  \tilde y, E_\ell y\rangle =\sum_{k\in\mathbb{Z}} \imag k \tilde y_k y_k =0,
\end{equation}
with $\tilde y$ an approximation of the solution.

Similar to the Hopf bifurcation validation presented in \cite{BLQ},  we  use a blow up approach in the neighborhood of a Hopf bifurcation. To this end, we  rewrite the solution $u\in\ELL$ to \eqref{e:full_KSF}  in the neighborhood of a Hopf bifurcation as the sum of the stationary solution $y\in \Ell$ to \eqref{e:eq_y} and a perturbation $az$, with amplitude $a\in\mathbb{R}$ and $z\in\ELL$ of order 1, that is
\begin{equation}\label{e:blowed_up}
\begin{cases}
u = E_{\ell} y + az,\\
%\| z\|_{\ELL}^2 = 1,
\langle \J^2 \overline{\tilde{z}},z \rangle = 1 ,
\end{cases}
\end{equation}
with $\tilde z$ a numerically determined approximation of $z$.
%
% where 
The second equation ensures that 
%$\|az\|_{\ELL}=|a|$, that is, $a$ is the amplitude of $az$, and 
$z$ does not tend to a (singular) stationary orbit as the Hopf bifurcation point is approached.
%
% However, we are not interested in computing precisely the norm of $z$; we are just interested in imposing a non-degeneracy condition on $z$. Therefore we replace the second equation with the easier to compute
% $$
% \langle \J^2 \overline{\tilde{z}},z \rangle - 1 =0,
% $$
%with $\tilde z$ a numerically determined approximation of $z$.

Replacing $u$ in \eqref{e:full_KSF} by $E_{\ell} y + az$, we arrive at
\begin{equation}
\begin{cases}
\langle \J^2\overline{\tilde{z}},z\rangle = 1,\\
\langle\imag \K  (E_{\ell} \tilde y+\tilde a\tilde z),( E_{\ell} y+az)\rangle = 0,\\
\langle\imag \J  (E_{\ell} \tilde y+\tilde a\tilde z),( E_{\ell} y+az)\rangle = 0,\\
\imag \J (E_{\ell} y+az)  +\lambda_1\lambda_2  \K^4 (E_{\ell} y+az) \\
\hspace{1cm}- \lambda_1 \K^2 (E_{\ell} y+az) -  \lambda_1\imag \K ((E_{\ell} y+az) * (E_{\ell} y+az)) =0.\\
\end{cases}
\end{equation}
We add the equations \eqref{e:eq_y} and \eqref{e:pc_y} and use this information on $y$ to simplify the terms involving only $y$ in the last equation. Concerning the phase condition in time, we  recall that $y$ is time-independent, hence $\J y=0$. Following a division by $a$, 
we consider the zero-finding problem
\begin{equation} \label{e:HopfKS_old}
\begin{cases}
\langle \J^2\overline{\tilde{z}},z\rangle  -1=0,\\
\langle\imag \K  \tilde y, y\rangle_\ell =0,\\
\langle\imag \K  (  E_\ell \tilde y + \tilde a \tilde z), z\rangle =0,\\
\langle\imag \J  \tilde z,z\rangle =0,
\\
\lambda_2  \K^4 y -  \K^2 y - \imag \K (y * y)=0,\\
\imag \J z  +\lambda_1\lambda_2  \K^4 z - \lambda_1 \K^2 z -  \lambda_1\imag \K (2E_{\ell} y * z+az*z  )=0.\\
\end{cases}
\end{equation}

\begin{remark}
The equation $\langle\imag \K  (  E_\ell \tilde y + \tilde a \tilde z), z\rangle =0$ is not the only choice for the phase condition on $z$. Other choices are possible, such as setting $\langle\imag \K  \tilde z, z\rangle =0$. In particular, the choice made in this paper is unfit in case $y$ is a homogeneous steady state, because in that case the equation would be trivially satisfied at the bifurcation point. However, in the case at hand $y$ is space-dependent, hence the stated condition is appropriate.
\end{remark}


%Furthermore, in order to simplify the phase conditions presented in \eqref{e:HopfKS_old}, we want to linearise them by replacing one of the two unknowns with a numerical approximation of it. 
Let $\hat x = (\hat \lambda_1,\hat\lambda_2,\hat a,\hat y, \hat z)$ be a numerical approximation of the solution of \eqref{e:HopfKS_old}, with $\hat y$ and $\hat z$ having just a finite number of non-zero Fourier coefficients. We use the numerical approximation to fix the phase conditions. The problem can then be written as
\begin{equation}\label{e:HopfKS}
\begin{cases}
&G^{\hat x} (\lambda_1,\lambda_2, a, y,z) =\begin{pmatrix}
\langle \J^2\overline{\hat{z}},z\rangle  -1\\
\langle\imag \K  \hat y,  y\rangle_\ell \\
\langle\imag \K ( E_{\ell} \hat y+\hat a\hat z),z\rangle \\
\langle\imag \J  \hat z,z\rangle \end{pmatrix}= 0,\\
&F(\lambda_1,\lambda_2, a, y,z) =\begin{pmatrix}
F_1(\lambda_2,y)\\
F_2(\lambda_1,\lambda_2, a, y,z )\\
\end{pmatrix} = 0.
\end{cases}
\end{equation}
Here we have split the problem into a linear problem $G^{\hat x}$, where we emphasize the dependency on the numerical approximation, and a nonlinear problem $F$, with $F_1$ as defined in \eqref{e:eq_y}  and 
$$
F_2(\lambda_1,\lambda_2, a, y,z)  \bydef \imag \J z  +\lambda_1\lambda_2  \K^4 z - \lambda_1 \K^2 z -  \lambda_1\imag \K (2E_{\ell} y * z+az*z)  . 
$$

We will at times use the notation $(F_1)_k$ and $(F_2)_{jk}$ to indicate the $k$-th and $(j,k)$-th Fourier coefficients of $F_1(x)$ and $F_2(x)$ respectively, where the argument will be clear from context.

The set of variables for \eqref{e:HopfKS} has the form $(\lambda_1,\lambda_2, a, y,z )$ with $\lambda_1,\lambda_2, a\in\mathbb{C}$, $y\in \ell^1_{\nu_2}$ and $z\in\ELL$. The full space of variables is thus
\begin{equation}\label{e:X_def}
X \bydef \mathbb{C}^3\times\ell^1_{\nu_2}\times\ELL,
\end{equation}
equipped with the product norm
$$
\|x\|= \|(\lambda_1,\lambda_2, a, y,z )\| \bydef \max\{ |\lambda_1|,|\lambda_2|,| a|,\| y\|_{\ell^1_{\nu_2}},\|z\|_{\ELL} \}.
$$
At times, we will also use the so-called component norm
\begin{equation}\label{e:c_norm}
\|x\|_c\bydef ( \max\{|\lambda_1|,|\lambda_2|,| a|\},\| y\|_{\ell^1_{\nu_2}},\|z\|_{\ELL} )\in\mathbb{R}^3.
\end{equation}


% === conjugate symmetry
\begin{definition}
The conjugate $x^*$ of $x\in X$ is defined by
\begin{equation*}
x^* \bydef (\bar\lambda_1,\bar\lambda_2, \bar a, y^*,z^*),\\
\end{equation*}
with the conjugate of $y$ and $z$ defined by
\begin{align*}
&y^*_k \bydef \bar y_{-k},\quad k\in\mathbb{Z},\\
&z^*_{jk} \bydef \bar z_{-j-k}, \quad j,k\in\mathbb{Z}.
\end{align*}
Let $Y$ be a space on which conjugate symmetry is defined, such as $X$,  $\Ell$,  or $\ELL$. Then the subspace of conjugate symmetric elements is denoted by $$\mathcal{S}(Y) \bydef \{ x\in Y: x = x^*\}.$$
\end{definition}

\begin{definition}\label{symm_op}
A map $T:X\rightarrow X$ is said to preserve conjugate symmetry if $T(\mathcal{S}(X) ) \subseteq \mathcal{S}(X) $.
\end{definition}
% == 
For $\nu'<\nu$, we have
\begin{align*}
\begin{pmatrix}
G^{\hat x}\\F
\end{pmatrix}:\mathbb{C}^3\times\ell^1_{\nu_2}\times\ELL &\rightarrow \mathbb{C}^4\times\ell^1_{\nu_2'}\times\ELL[\nu']\\
(\lambda_1,\lambda_2,a,y,z)&\mapsto (v',y',z').
\end{align*}
Furthermore, $(F_1)_k$ and $(F_2)_{jk}$ vanish for $k=0$ and $(j,k) = (0,0)$, that is $y_0' = 0$ and $z_{00}'= 0$. Therefore we can compose with the map
\begin{align*}
\tilde \Pi :\mathbb{C}^{n}\times\ell^1_{\nu_2'}\times\ELL[\nu'] &\rightarrow \mathbb{C}^{n-2}\times\ell^1_{\nu_2'}\times\ELL[\nu'] \\
(v',y',z')&\mapsto(v'',y'',z'')
\end{align*}
 with $v''_i = v'_i$ for $i = 1,\dots, n-2$
and
$$
y''_k = \begin{cases}
v'_{n-1} &\text{if } k = 0,\\
y'_k\quad & \text{if } k\neq 0,\\
\end{cases} \quad \text{and} \quad 
z''_{jk} = \begin{cases}
v'_n &\text{if }(j,k)= (0,0),\\
z'_{jk}\quad & \text{if } (j,k)\neq (0,0).
\end{cases}
$$
%The corresponding embedding is denoted by $\tilde E$. 
In this way we remove the trivial identities from the formulation and arrive at 
\begin{equation}\label{e:H}
H^{\hat x}(x) \bydef \tilde\Pi \begin{pmatrix}
G^{\hat x}\\F
\end{pmatrix}(x) =0,
\end{equation}
which generically has a one-dimensional solution set.
We abuse notation by not specifying $n=4$ in the definition of $\tilde \Pi$, so that we can reuse the notation later in a slightly more general setting.

%==%



Let $x = (\lambda_1,\lambda_2, a, y,z )\in X$ and $w = (\beta_1, \beta_2, b,r,s)\in X$, then we extend the notation $\langle \cdot ,\cdot\rangle$ to $X$ by defining
$$
\langle x, w\rangle \bydef \lambda_1\beta_1 +\lambda_2\beta_2+ab+ \langle  y,  r\rangle_\ell + \langle z,s\rangle.
$$ 

In the following, we will assume we have computed two numerical solutions $\hat x_0 = (\hat \lambda_{10},\hat\lambda_{20},\hat a_0,\hat y_0, \hat z_0)\in\mathcal{S}(X)$ and $\hat x_1= (\hat \lambda_{11},\hat\lambda_{21},\hat a_1,\hat y_1, \hat z_1)\in\mathcal{S}(X)$ of \eqref{e:HopfKS}. Assuming the two numerical solutions are close to each other, i.e. $\| \hat x_0 - \hat x_1\| \ll 1$, it is reasonable to expect that the segment connecting them is an approximation of a nearby solution branch. To construct a one-to-one correspondence between the point on the segment $[\hat x_0,\hat x_1]$ and the solution branch $x(s)$, $s\in[0,1]$, we follow \cite{JP} and add to \eqref{e:HopfKS} the so-called continuation equation 
\begin{equation}\label{e:cont_eq}
\Es(x) = \langle x, q_s\rangle - c_s,
\end{equation}
where
$$
q_s = q_0 + s(q_1 - q_0), \qquad \text{ and } \qquad c_s = c_0  + s(c_1-c_0),
$$
with %\red{add statement on new continuation}
\begin{equation}\label{e:cont_eq_coefs}
q_\s =( v_\s+v_\s^*)/2, \qquad \text{ and } \qquad c_\s = \langle  \hat x_\s,q_\s\rangle, \qquad\text{ for } \s = 0,1,
\end{equation}
where  $v_\s$ is approximately in $\ker(DH^{\hat x_\s}(\hat x_\s))$, with $H^{\hat x_\s}(x) $ defined in \eqref{e:H}. Furthermore, we assume $q_\s$, for $\s = 0,1$, has finitely many non-zero Fourier coefficients, as do $\hat x_0$ and $\hat x_1$. The continuation problem is then
%\begin{equation} 
% \begin{pmatrix}
%\Es(\lambda_1,\lambda_2, a, y,z) \\
%G^{\hat x_s}(\lambda_1,\lambda_2, a, y,z) \\
%F(\lambda_1,\lambda_2, a, y,z) 
%\end{pmatrix}=0.
%\end{equation}
%Then, we set
\begin{equation}\label{e:HopfKS_cont}
H_s(\lambda_1,\lambda_2, a, y,z) = \tilde \Pi \begin{pmatrix}
\Es(\lambda_1,\lambda_2, a, y,z) \\
G^{\hat x_s}(\lambda_1,\lambda_2, a, y,z) \\
F(\lambda_1,\lambda_2, a, y,z) 
\end{pmatrix}.
\end{equation}


\begin{remark}
It follows from the definition of $H_s$ in \eqref{e:HopfKS_cont} that
$$
H_s(x^*) = H_s(x)^*, 
$$
where the codomain of $H_s$ is $ X' = \mathbb{C}^3\times \Ell[\nu_2']\times \ELL[\nu']$ for $\nu' <\nu$. Therefore,  $H_s$ preserves conjugate symmetry.
\end{remark}


We are interested in solving the continuation problem
\begin{equation}\label{e:Hs}
H_s:X\rightarrow X', \qquad H_s(x) =0\quad \text{for all } s\in [0,1].
\end{equation}

\begin{remark}\label{r:is_Hopf}
A solution branch $x(s)$ of \eqref{e:Hs} goes through a Hopf bifurcation if there exist $s^*,s_0$ and $s_1$ such that $s^*\in (s_0,s_1)$, $a(s^*)=0$ and $a(s)\neq 0$ for $s\in[s_0,s_1]\backslash \{s^*\}$. The latter statement guarantees that the time-dependent term $az$ does not vanish unless $a=0$.

By continuity of $a(s)$, if it holds that $a(s_0)\cdot a(s_1)<0$ then there exists a $s^*\in (s_0,s_1)$ such that $a(s^*)=0$.  We are thus left with proving that $a(s)$ changes sign along the validated solution branch and $a'(s^*)\neq 0$, in order to prove the existence of a Hopf bifurcation of the Kuramoto-Sivashinsky equation.
%Let $x(s)$ be the solution branch of \eqref{e:Hs}, then if there is a unique $s^*$ such that $a(s^*)=0$, then a Hopf bifurcation is taking place at $s=s^*$. 
%
%Furthermore, if $a$ is monotone and changes sign between $s=0$ and $s=1$, i.e. it holds $a(0)\cdot a(1) < 0 $, then a Hopf bifurcation is taking place at some value $s^*\in [0,1]$. 
\end{remark}


\begin{remark}\label{r:cont_eq}
%\red{If $q_\s$ is chosen to vanish every}
Although we have formulated the problem in the context of general pseudo-arclength continuation, 
we can choose the continuation equation~\eqref{e:cont_eq}  to conveniently simplify the verification in Remark~\ref{r:is_Hopf}. Indeed, the choice
% There is another possible choice for the continuation equation $\Es$. We can chose to use it to impose parameter continuation. In this specific case, we want to follow the parameter $a$, thus we define
% $$
% \Es (x) = a - \hat a_s.
% $$
% In the notation used in \eqref{e:cont_eq}, this is equivalent to chose
$$
q_\s = (0,0,1, 0,0)\in X \qquad \text{and}\qquad c_\s = \hat a_\s
$$
in essence turns the general (pseudo-arclength) continuation into parameter continuation with respect to $a$. 
In this case, if a solution exists,  we immediately conclude that $a'(s)\neq 0$, provided $\hat{a}_0 \neq \hat{a}_1$. As a consequence, if $\hat{a}_0  \cdot\hat{a}_1<0$, we can prove that $a(s)$ changes sign along the validated curve of solutions and Remark~\ref{r:is_Hopf} implies the existence of a Hopf bifurcation.
 % we prove the existence of a non-degenerate Hopf bifurcation, as follows from Remark \ref{r:is_Hopf}.
\end{remark}


%</problem>






==> radii_pol.tex <==
%<*radii-pol>

For the parameter dependent zero finding problem \eqref{e:Hs}, we aim to validate the segment between two numerical solutions $\hat x_0$ and $\hat x_1$, %The numerical solutions are such that
which are such that
$$
H_\s(\hat x_\s)\approx 0, \quad \hat x_\s\in \mathcal{S}(X)\quad \text{for } \s=0,1.
$$
For $s\in [0,1]$, we introduce the notation
$$
\hat x_s = \hat x_0 + s(\hat x_1-\hat x_0).
$$


Following \cite{JP}, we transform the zero finding problem \eqref{e:Hs} into a parameter dependent fixed point problem
$$
T_s(x) = x,
$$
with $s\in [0,1]$ and $T_s$ the Newton-Kantorovich operator defined by
\begin{align}\label{e:defT}
T_s:X&\rightarrow X\\
x&\mapsto x-A_sH_s(x),
\end{align}
where $A_s$ is an approximation of $DH_s(\hat x_s)^{-1}$ for all $s$ in $[0,1]$. The linear operator $A_s$ will be constructed in Section \ref{s:bounds} satisfying the following conditions:
\begin{align} \label{conditions_A}
\begin{split}
& A_sH_s(x)\in X \text{ for }x\in X\\
& A_s \text{ is injective for all }s\in [0,1].
\end{split}
\end{align}

In order to prove that $T_s$ is a contraction in a neighborhood of $\hat x_s$, we first introduce 
%the notation for a cylinder of radius $r$ along $\hat x_s$ in $X$, that is
%$$
%\mathcal{C}_ r \bydef \bigcup_{s\in [0,1]} B_r(\hat x_s),
%$$
%where
$$
B_r( x) \bydef \left\{ 
y\in X : \|y-x\|_X \leq r
\right\}.
$$
To prove that $T_s$ is a contraction in $B_r(\hat x_s)$ for some $r$, we determine bounds
\begin{equation}\label{e:Y_bound}
Y_s \geq \max_{s\in[0,1]}\| T_s(\hat x_s) - \hat x_s\|_X,
\end{equation}
and
\begin{equation}\label{e:Z_bound}
Z_s(r) \geq \max_{s\in[0,1]}\sup_{b,c \in B_1(0)\subset X}\| DT_s(\hat x_s+rb) rc\|_X.
\end{equation}
With $Y_s$ and $Z_s(r)$ computed rigorously, we can then apply the following parame\-trized Newton-Kantorovich theorem and validate our numerical approximations.

\begin{theorem}\label{t:rad_poly}
Let $A_s$ satisfy the condition \eqref{conditions_A}, let $T_s:X\rightarrow X$ be defined as in \eqref{e:defT}, let $Y_s$ and $Z_s(r)$ be defined as in \eqref{e:Y_bound} and \eqref{e:Z_bound} respectively. Let the radii polynomial be defined as
$$
p(r) \bydef Y_s + Z_s(r)-r.
$$
If there exists an $r^*>0$ such that
$
p(r^*)<0
$
then there exists a continuous curve $\{x(s)\}_{s\in[0,1]}\subset X$ such that $x(s)\in B_{r^*}(\hat x_s)$ and $H_s(x(s))=0$ for all $s\in [0,1]$. Furthermore, if $\hat x_\s,q_\s\in\mathcal{S}(X)$, then  $x(s)\in\mathcal{S}(X)$.
\end{theorem}
\begin{proof}
The first part of this Theorem has been presented and proven in many contexts, such as in \cite{JP} and \cite{QJBcontinuation}.

The symmetry argument follows from the following considerations. Thanks to the injectivity of $A_s$, $T_s(x(s)) = x(s)$ implies $H_s(x(s)) = 0$. We have $H_s(x(s))^* = H_s(x(s)^*) = 0$ and thus $T_s(x(s)^*) = x(s)^*$. Since $\hat x_s\in\mathcal{S}(X)$, the ball $B_{r^*}(\hat x)$ is invariant under conjugate symmetry, hence $x(s)^*\in B_{r^*}(\hat x)$. Due to uniqueness of the fixed point of $T_s$ in $B_{r^*}(\hat x)$, we conclude that $x(s)^* = x(s)\in \mathcal{S}(X)$.
\end{proof}

When the continuation equation is chosen as in Remark \ref{r:cont_eq}, then the solution curve $\{x(s)\}_{s\in[0,1]}\subset X$ is smooth.



%</radii-pol>


==> symmetry.tex <==
%<*symmetry>

%\blue{This section is a mess. Working on it.}
%\red{Elena: where is the definition of symmetry preserving $A$?}

Since we are looking for real-valued periodic solutions of the ODE~\eqref{e:main}, its Fourier coefficients are conjugate symmetric in the following sense.
%we are mainly interested in Fourier sequences corresponding to real valued functions. This is equivalent to request the Fourier sequence to be conjugate symmetric, as introduced in the next Definition.
%\begin{definition}
For $w \in \ell^1_\nu$ we define the conjugate $w^*$ as $w^*_{k} = \overline{w_{-k}}$. An element $w\in \ell^1_\nu$ is conjugate symmetric if  $w =w^*$. We denote the space of conjugate symmetric sequences by $\ellsym_\nu=\{w\in \ell^1_\nu : w =w^*\}$. With this definition, periodic orbits have Fourier coefficients $u_n \in \ellsym_\nu$ for all $n=1,\dots,N$ and some $\nu>1$.
%This definition deals with the Fourier sequences, w

We generalize this notation of conjugation to $\XX$ by setting 
\[
x^* = (\lambda,v)^* = (\overline{\lambda_1},\dots,\overline{\lambda_M},v_1^*,\dots,v_N^*) .
\]
We introduce the space of (conjugate) symmetric elements $\SSS\subset \XX = \C^M \times (\ell^1_\nu)^N$:
\begin{equation}\label{calliS}
\SSS = \SSS_\nu \bydef \{x  \in \XX : x^*=x \}.
\end{equation}
We look for a solution in this space of (conjugate) symmetric elements, and we will also choose our numerical approximation in $\SSS$. Nevertheless, we use the full space to perform our validation proof because of the ease of performing analysis on unrestricted double sided convolutions. In particular, we do not restrict to symmetric cases where sine or cosine series can be used. Such cases have been studied extensively, see  e.g.~\cite{BLchaos,breden-vanicat,castelli-breden,hungria-lessard,LMRansford}.  Furthermore, we do not split into real and imaginary parts (cf.~\cite{Ldelay}) but rather recover conjugate symmetry a posteriori using the symmetry properties discussed below.

We now derive the results needed to prove that the fixed point of $T_s$ found in Theorem~\ref{radii_bound} lies in $\SSS$, provided we choose a symmetry preserving linear operator $A_s$ in the definition~\eqref{e:defTs} of $T_s$. First we note that $\ellsym_\nu$ is closed under convolution multiplication. Moreover, for any $x=(\lambda,v)\in \SSS$ any polynomial expression in $v$ with real coefficients (depending on $\lambda \in \R^M$) also lies in $\SSS$. Choosing both $\hat{q}_{\s} \in \SSS$ and $\dot{\hat{x}}_{\s} \in \SSS$ for $\s=0,1$, we infer that $G^\phase_s$ and $G^\cont_s$ are real-valued  on $\SSS$ for all $s\in [0,1]$, since the bilinear form defined in~\eqref{e:bilinear} sends $\pi_K \SSS \times \pi_K \SSS$ to $\mathbb{R}$. We conclude that $H_s$ maps $\SSS_\nu$ to $\SSS_{\nu'}$ for $1<\nu'<\nu$.

Next, we choose the linear operators $A_0$ and $A_1$ such that they (and hence $A_s$ for $s\in [0,1]$) preserve symmetry in the sense that they leave $\SSS$ invariant. This impies that $T_s$ maps $\SSS$ to itself for all $s\in [0,1]$. To be explicit, for a linear operator $B=(B_{nm})$ on $\XX$ we introduce the conjugate $B^*$ as follows ($k,k' \in \Z$):%
\begin{subequations}
\label{e:conjugate}
\begin{alignat}{2}
    B^*_{nm} &= \overline{B_{nm}} && \quad\text{for } n,m=1,\dots,M , \\
    (B^*_{nm})_{k} &= \overline{(B_{nm})_{-k}} && \quad\text{for } m=1,\dots,M , n=M+1,\dots,M+N,\\
    (B^*_{nm})_{k} &= \overline{(B_{nm})_{-k}} && \quad\text{for } n=1,\dots,M , m=M+1,\dots,M+N, \\
    (B^*_{nm})_{k,k'} &= \overline{(B_{nm})_{-k,-k'}} && \quad\text{for } n,m=M+1,\dots,M+N.
\end{alignat} 
\end{subequations}
Then $A_{\s}$, $\s=0,1$ preserves conjugate symmetry if $A_{\s}=A_{\s}^*$.

\begin{remark}\label{r:symmetricA}
Since $i\boldsymbol{K}^{-1}$ preserves conjugate symmetry, conjugate symmetry preservation of $A_{\s}$ in practice reduces to symmetry preservation of the approximate numerical approximate inverse of $D\hat H_{\s}(\hat{x}_{\s})$. Due to rounding error in computing the numerical inverse, this symmetry is not automatic. We therefore symmetrize the candidate inverse, denoted by $\tilde{A}_{\s}$, through 
$$
\hat{A}_{\s} = \frac{\tilde{A}+\tilde{A}^*_{\s}}{2},
$$
with the conjugate defined in~\eqref{e:conjugate}.
% \red{Elena: what it the definition of putting the bar over such an operator?}
% Since $\imag \boldsymbol{K}^{-1}$ preserves conjugate symmetry, the full operator $A$ then preserves conjugate symmetry.
%where$\tilde{\hat{A}}$ is a first numerical inverse of $D\hat H(\hat x)$
\end{remark}

 
The symmetries thus allow us to conclude that the fixed point of $T_s$ correspond to a \emph{real}-valued periodic orbit of~\eqref{e:main} under symmetry assumptions on the numerical data. In particular, in practice we fix some $K \in \mathbb{N}$ and choose
%\red{Elena: this is done in the code now? yes}
\begin{itemize}
\item
 the numerical approximate solutions $\hat{x}_0$ and $\hat{x}_1$ in $\Pi_K \SSS$;
\item
 the numerical predictors $\dot{\hat{x}}_0$ and $\dot{\hat{x}}_1$ in $\Pi_K \SSS$;  
\item
 the phase condition parameters $\hat{q}_0$ and $\hat{q}_1$ in $\Pi_K \SSS$,
 see~\eqref{e:choiceq};
\item
 conjugate symmetry preserving linear operators $\hat{A}_0$ and $\hat{A}_1$, see Remark~\ref{r:symmetricA}. 
\end{itemize}
 
 
% We will here investigate what actions are we allowed to take while preserving complex conjugacy and  how we can prove that the exact solution in the $\ell^1_\nu$ space corresponds to a real orbit.
%Therefore, we would like to study how the operations we are carrying out affect this symmetric space. In particular, the following Lemmas hold.
%We also introduce the notation $x=(a,v)\in \mathcal{S}\subset \mathbb{C}^M\times (\ell^1_\nu)^N$  if $v_i\in \ellsym$ for $i=1,\dots,N$ and $\overline{a}=a$, i.e. $a\in\mathbb{R}$.

% \begin{lemma}\label{convolution_preserves_sym} The convolution of two sequences in  $\ellsym_\nu$ is again a sequence in  $\ellsym_\nu$. Moreover, for any $x=(\lambda,v)\in \SSS$ any polynomial expression in $v$ with real coefficients (depending on $\lambda \in \R^M$) also lies in $\SSS$.
% %\blue{Removed notation for powers.}
% %** should I say something about the application of $\imag k$ to $x$? probably...
% \end{lemma}
% \begin{proof}
% 	To prove the first assertion, let $v,w\in  \ellsym_\nu$ and $y=v\cdot w$,
% 	then
% $$
% y_{-k} =  \! \! \!\sum_{k_1+k_2=-k} \! \! \!v_{k_1}w_{k_2} =  \sum_{k_1+k_2=k}  \!  \! v_{-k_1}w_{-k_2} =\sum_{k_1+k_2=k} \overline{v}_{k_1}\overline{w}_{k_2}=\overline{y}_k .
% $$
% It is easy to see that this generalizes to convolutions of any order, since convolutions are associative, and the second assertion follows.
% \end{proof}

% We would like the map $T_s$ to preserve conjugate symmetry, and the following Lemma \ref{linear_operators_preserve_sym} and  Corollary \ref{real_requests} give sufficient conditions for this.
% % something about the operator
% \begin{lemma}\label{linear_operators_preserve_sym}
% Considering a linear operator $B: \ell^1_\nu \rightarrow \ell^1_{\nu '}$, with
% $$
% Bx = y , \qquad y_k = \sum_{l\in \mathbb{Z}} B_{k,l} x_l,\qquad k\in\mathbb{Z},
% $$
% then $ \ellsym_\nu $ is mapped into $ \ellsym_{\nu'} $  under $B$ if and only if it holds
% \begin{equation}\label{e:Msym}
% B_{k,l} = \overline{B}_{-k,-l}, \qquad \text{for all } k,l \in \mathbb{Z}.
% \end{equation}
% \end{lemma}
% If $B$ satisfies~\eqref{e:Msym} we say that $B$ preserves conjugate symmetry.
% \red{Elena: but this way ``preserving conjugate symmetry'' is defined only for maps on $\ell^1_\nu$, not on $\XX$!}
% The proof of Lemma~\ref{linear_operators_preserve_sym} is analogous to that of Lemma~\ref{convolution_preserves_sym}, and the details are left to the reader.%\begin{definition}
%A linear operator $A:\ell^1_\nu\rightarrow\ell^1_\nu$ is called an conjugate symmetric** if it sends conjugate %sequences in conjugate sequences.
%\end{definition}
% The proof follows again by direct computation and will not be presented here.

% The equations $P_s=0$ represent the original system~\eqref{e:main} appended with a phase condition $G^\phase=0$ and continuation equation $G^\cont=0$.
% The definitions of these latter two functions in Section~\ref{s:phase} is based on coefficients $\hat{q}_i$ and $\dot{\hat{x}}_i$ as well as $\hat{x}_i$, for $i=0,1$.
% For the full problem to respect conjugate symmetry, the mentioned  coefficients need to be conjugate symmetric. Moreover, for the fixed point problem to preserve conjugate symmetry, the linear operator $A_s = (1-s) A_0 + sA_1$
% needs to preserve conjugate symmetry, which is guaranteed if both $A_0$ and $A_1$ do, since $\SSS$ is convex. This is summarized in the following corollary.
% \begin{corollary}\label{real_requests}
% Let $\emb\hat{q}_i, \emb\dot{\hat{x}}_i, \emb\hat{x}_i \in \SSS$
% for $i=0,1$. If $A_0$ and $A_1$ preserves conjugate symmetry, then $T_s$ preserves conjugate symmetry for every $s\in[0,1]$.
% \end{corollary}
% \begin{proof}
% %\red{JB: proof still needs to be  adapted to new notation.}
% The fixed point operator $T_s$ preserves conjugate symmetry if $A_s$ and $P_s$ preserve it. Since it follows directly from the assumptions that $A_s$ preserves conjugate symmetry, it remains to proves that $P_s$ does. We see from~\eqref{global_Ps} that $P_s$ preserves conjugate symmetry if, for any $x=(\lambda,v) \in \SSS$, we have $G_s(x)\in \mathbb{R}^{M}$ and $F(x)\in (\ellsym_{\nu'})^N$.
%
% We recall that $\lambda=(\tau,\mu)$.
% For the scalar part of $G$ it follows that $g(\mu) \in \mathbb{R}^{M-2}$, since $\mu \in \mathbb{R}^{M-1}$ for all $n=1,\dots,M-1$.
% For the continuation equation we have $G^\cont_s(x) \in \mathbb{R}$ for $x \in \SSS$, since
% it is assumed that  $\dot{\hat{x}}_i, \hat{x}_i \in \SSS$ for $i=0,1$, and  the bilinear form defined in~\eqref{e:bilinear} sends $\pi_K \SSS \times \pi_K \SSS$ to $\mathbb{R}$. An analogous argument, with $\dot{\hat{x}}_i$ replaced by $\hat{q}_i$, gives $G^\phase_s(x) \in \mathbb{R}$ for $x \in \SSS$.

% The functions $F_n$ consist of two parts, see~\eqref{F}. The second part,
% denoted by $\widehat{f}_n$ is a real convolution polynomial in $v$ for $\lambda \in \R^M$, hence $\widehat{f}_n(\lambda,v) \in \ellsym_\nu$ for all $\lambda \in
% \mathbb{R}^{M}$ and $v\in (\ellsym_\nu)^N$. Furthermore, it is not hard to
% check that the first part of $(F_n(x))_k$, which is given by $\imag\! k(v_n)_k
% $ sends $\ellsym_\nu$ to $\ellsym_{\nu'}$ for any $\nu'>\nu$. We conclude
% that $F$ preserves conjugate symmetry.

% the operator that we denote by $\imag\! \boldsymbol{k}$, that acts, for $v\in\ell^1_\nu$ as
% \begin{equation}\label{operator_k}
% \imag\! \boldsymbol{k} v = w\in \ell^1_{{\nu}'},  \qquad (w)_k = \imag\! k (v)_k, \qquad \text{for } k\in\mathbb{Z},
% \end{equation}
% This operator satisfy the hypothesis of Lemma \ref{linear_operators_preserve_sym}, hence both $\imag\! \boldsymbol{k}$ and $F$ preserve conjugate symmetry.
% %follows from the previous,

% Finally, we need to show that  $E_s(x)\in \mathbb{R}$ for $x \in \SSS$. This follows easily from the assumptions
% %
% We first remark that, if $\hat x_0,\hat x_1\in \SSS$, then $\hat x_s \in \SSS$, since $\SSS$ is closed under addition and real scalar multiplication.
%
% We then have to show $\langle x-\hat{x}_s , \dot{\hat{x}}_s\rangle \in \mathbb{R}$, or more in general $\langle x,y\rangle  \in \mathbb{R}$ for $x,y\in \SSS$, and it follows from direct computation:
% $$
% \langle x,y\rangle  = \sum_{n=1}^M x_n y_n + \sum_{n=M+1}^{N+M} \sum_{k=-\infty}^\infty (x_n)_k (y_n)_k,
% $$
% the first sum is a sum of real scalars, it is therefore in $\mathbb{R}$, in the second, for a fixed $n$ we consider
% $$
%  \sum_{k=-\infty}^\infty (x_n)_k (y_n)_k = (x_n)_0 (y_n)_0 + \sum_{k=1}^\infty \Big( (x_n)_k (y_n)_k + (x_n)_{-k} (y_n)_{-k}\Big),
% $$
% the first term is again trivially real, while for the infinite sum, considering term by term, we have
% $$
% (x_n)_k (y_n)_k + (x_n)_{-k} (y_n)_{-k} = (x_n)_k (y_n)_k + (\overline{x}_n)_{k} \,\, (\overline{y}_n)_{k}=(x_n)_k (y_n)_k + (\overline{x}_n)_{k} (\overline{y}_n)_{k}\in \mathbb{R}.
% $$
% This concludes the proof.
% \end{proof}

\begin{theorem}\label{t:symsol}
Let the symmetry assumptions on $\hat{x}_{\s}$, $\dot{\hat{x}}_{\s}$, $\hat{q}_{\s}$, $\hat{A}_{\s}$ listed above be satisfied for $\s=0,1$. 
Then, under the conditions of  Theorem~\ref{radii_bound}, the fixed point $x_\sol(s) \in B_{\widehat{r}}(x_s)$ of $T_s$ is conjugate symmetric, 
i.e.~$x_\sol(s) \in \SSS$, for every $s\in[0,1]$.
\end{theorem}
\begin{proof}
Since $\SSS$ is invariant under $T_s$ and it intersects $B_{\widehat{r}}(x_s)$, as $x_s \in \SSS$, the fixed point of $T_s$ lies in $\SSS \cap B_{\widehat{r}}(x_s)$.
\end{proof}

Theorem~\ref{t:symsol} provides us with $x_\sol(s) \in \SSS$, which we write as  $ x_\sol(s)= ((\tau_\sol,\mu_\sol),v_\sol)(s)$. We have thus found a family of real-valued solutions
\[
u_\sol (t;s) \bydef \sum_{k\in\mathbb{Z}} (v_\sol (s))_k  e^{\imag  k  t/ \tau_\sol(s) },
\]
of~\eqref{e:main} with period $L = 2\pi \tau_\sol(s)$ at parameter value $\mu=\mu_\sol(s) \in \R^{M-1}$.
We denote 
\[
  (1-s) \hat{x}_0 + s \hat{x}_1 = \hat{x}_s = (\hat{\lambda}_s,\hat{v}_s)
   = ((\hat{\tau}_s,\hat{\mu}_s),\hat{v}_s),
\]
so that $x_s = \emb \hat{x}_s \in \SSS$, see~\eqref{definition_xs}.
\begin{remark}\label{r:errorbound}
Since $x_\sol(s) \in B_{\widehat{r}}(\emb \hat{x}_s)$, the associated error estimates are 
\begin{alignat}{1}
  \max_{t\in \mathbb{R}} \left|u_\sol (t;s)  - \hat{u}_s \bigl( \tfrac{\hat{\tau}_s}{\tau_\sol(s)} t\bigr) \right|_\infty  & \leq \widehat{r}, \label{e:errorestimate} \\
   |\tau_\sol(s) - \hat{\tau}_s|  &\leq \widehat{r}, \nonumber \\
   |\mu_\sol(s) - \hat{\mu}_s|_\infty  &\leq \widehat{r}, \nonumber
\end{alignat}
for all $s \in [0,1]$,
where %\red{This sum needs to be finite: $|k| \leq K$}
\[ 
  \hat{u}_s (t)  \bydef \sum_{|k| \leq K} (\hat{v}_s)_k  e^{\imag  k t/ \hat{\tau}_s }.
\] 
In particular, the bound \eqref{e:errorestimate} implies that for any $s\in [0,1]$  the periodic orbit $u_\sol(\cdot;s)$ lies within Hausdorff distance $\widehat{r}$ from the closed curve $\hat{u}_s(\cdot)$ in phase space (in the supremum norm). 
\end{remark}

%</symmetry>


==> symmetry_considerations.tex <==
%!TEX root = HopfKS.tex

While validating the numerical solution $\hat x = (\hat \lambda_1, \hat\lambda_2,\hat a, \hat y, \hat z)$ to \eqref{e:HopfKS}, we also want to prove that the associated solution in the phase space is real. This is equivalent to request
\begin{align*}
\lambda_1,\lambda_2,a&\in \mathbb{R},\\
y\in \ell^1_\nu &:y_k e^{\imag k x} +  y_{-k}e^{-\imag k x} \in\mathbb{R},\\
z\in\ELL &: z_{jk} e^{\imag j t+\imag k x} +  z_{-jk} e^{-\imag j t+\imag k x} +  z_{j-k} e^{\imag j t-\imag k x} +  z_{-j-k} e^{-\imag j t-\imag k x}\in\mathbb{R}
\end{align*}
The second request corresponds to 
$$
y\in \ell^1_\nu : y_k = \bar y_{-k},
$$
while the third is encapsulated in 
$$
z\in \ELL:  z_{jk} = \bar   z_{-j-k}.
$$
We therefore introduce the conjugate symmetric spaces
$$
\mathcal{S}(\ell^1_\nu) = \{ y\in \ell^1_\nu : y_k = \bar y_{-k}\},
$$
and
$$
\mathcal{S}(\ELL) = \{ z\in \ELL:  z_{jk} =  \bar z_{-j-k}\},
$$
and coherently 
\begin{equation}\label{symm_X}
\mathcal{S}(X) = \mathbb{R}^3\times \mathcal{S}(\ell^1_\nu) \times\mathcal{S}(\ELL) .
\end{equation}

We call elements of $\mathcal{S}(X) $ conjugate symmetric and we introduce the following definition.









==> tail.tex <==

%<*tail>
This section is devoted to bound the norm of some eventually diagonal operators, where we add some constraint on the diagonal part of the operator. Let $P$ be an eventually diagonal operator in $B(\ELL,\ELL)$ of center dimension $K = (M,N)\in\mathbb{N}^2$, then it has the form
\begin{align}\label{e:P}
P:\ELL &\rightarrow \ELL\\\nonumber
u&\mapsto P: (Pu)_{jk} = \begin{cases}
E(B \tau_2^{K}u)_{jk} &\text{for }(j,k)\in \F,\\
\mathbf{p}(j,k) u_{jk} \qquad &\text{otherwise,}\\
\end{cases}
\end{align}
for a function $\mathbf{p}$ and a matrix $B\in \mathbb{C}^{(2M+1)(2N+1)\times(2M+1)(2N+1)}$, see Remark~\ref{r:dim_fin_op}. In this section we will study the norm of $P$ when  $\mathbf{p}$ is a rational polynomial of the form 
\begin{equation}\label{e:p}
\mathbf{p}(j,k) = \frac{q(j,k)}{p(j,k)} =  \frac{q_1(j)+q_2(k)}{\imag p_1(j)+p_2(k)},
\end{equation}
with $p_1(j)$ and $p_2(k)$  real-valued polynomials and $q_1(j)$ and $ q_2(k) $ complex polynomials. If there is any constant term in $q$, it will be assigned to $q_2$. 

It  holds, by Lemma \ref{l:eventual_diag} and by the definitions of the operator norms in \eqref{e:sub_norm}, that
$$
\|P\| = \max\{\|B\|, \sup_{(j,k) \notin \F}  |\mathbf{p}(j,k)|\}.
$$

\begin{remark}
The bound on $ \sup_{(j,k) \notin \F}  |\mathbf{p}(j,k)|$  can be finite only if the order of $q_i$ is smaller than or equal to the order of $p_i$, 
for $i = 1,2$.
\end{remark}


To simplify the presentation, we will further restrict ourselves to 
$
p_1(j) = j
$,
although the 
results can be generalised to polynomial $p_1(j)$.
%, but it will go beyond the scope of this presentation.

By the triangle inequality
\begin{align}\label{e:triangleqp}
\sup_{(j,k) \notin \F } |\mathbf{p}(j,k)| &\leq \sup_{(j,k) \notin \F }  \left|\frac{q_1(j)}{\imag j+p_2(k)}\right| + \sup_{(j,k) \notin \F }  \left|\frac{q_2(k)}{\imag j+p_2(k)}\right|
\end{align}
 We will  consider the two fractions separately. With the restrictions imposed on~$q_1$, we have 
$
q_1(j) =  c_1 j.
$
Therefore the first fraction is bounded trivially by~$|c_1|$.
\begin{remark}\label{r:restriction}
If there exists a $(j^*,k^*)\notin F_K$ such that $p(j^*,k^*) = 0$, then the norm of $P$ is infinite. 
%Obviously,  $j^* =0$, 
Hence in the following we want to ensure that there is no $k^*\in\mathbb{N}$, such that $|k^*|>N$ and $p(0,k^*)=0$. This is incorporated in the definition of $Q_N$ in \eqref{e:bound_tail} below, which will simply be infinity if this is violated.%checked by Equation \eqref{e':vert_asympt}.
%\red{redo}
%If there exists a $(j^*,k^*)\notin F_K$ such that $p(j^*,k^*) = 0$, then the norm of $P$ is infinite. Obviously, it would hold that $j^* =0$. To avoid $p_2(k^*)= 0 $ for some $|k^*|>N$, we assume
%$$
% N>|k^*|,
%$$
%with $k^*\in\mathbb{N}$ the biggest integer solution of $p_2(k) =0$.
%The choice of $N$ will follow naturally by the algorithm explained below. \blue{In particular, we remark that the following algorithm does not require this assumption, but returns an infinite bound if it is not satisfied.}
%\red{we need this otherwise the norm of $P$ is infinite, but there is no way in checking it unless it's checked by the algorithm later on, how can I say it nicely?}
\end{remark}


Concerning the second term in the righthand side of~\eqref{e:triangleqp}, we remark that, for fixed $k$, 
$\left|\frac{q_2(k)}{\imag j+p(k)}\right|$ decreases if $|j|$ increases, hence
\begin{align}\label{e:fraction_split}
\sup_{(j,k) \notin \F } \left|\frac{q_2(k)}{\imag j+p_2(k)}\right|\leq \max \left\{ 
\max_{|j| = M+1, |k| \leq N+1} \left|\frac{q_2(k)}{\imag j+p_2(k)}\right|, \sup_{|k|>N} \left|\frac{q_2(k)}{p_2(k)}\right|
\right\}.
\end{align}
The first maximum of \eqref{e:fraction_split} is  taken over a finite set, hence  it is directly computable. The supremum, on the other hand, is computed over an infinite set and requires a more refined approach, i.e.,  
we want to bound 
\begin{equation}\label{e:two_star}
\sup_{|k|>N}\left| \frac{q_2(k)}{p_2(k)} \right|
\end{equation}
using a finite number of computations. As a first step, we construct $k'_1\in\mathbb{N}$
% as the integer upper bound of all vertical asymptotes, 
satisfying
\begin{equation}\label{e:vert_asympt}
p_2(x) \neq 0\quad \text{for all }|x|>k'_1,
\end{equation}
and 
%an integer upper bound 
$k_2'\in\mathbb{N}$ 
%on all local maxima and minima, 
satisfying
\begin{equation}\label{e:max_and_min}
q_2'(x)p_2(x) - p_2'(x)q_2(x) =0\quad \text{for all }|x|>k'_2. 
\end{equation}
To find $k_1$ and $k_2$, we use the minimum of Lagrange's and Cauchy's bounds, which provide explicit finite bounds on roots of polynomials. Then we set $k' = \max\{ k_1',k_2'\}$.

It then holds that \eqref{e:two_star} is bounded by
\begin{align}\label{e:bound_tail}
\begin{split}Q_N\bydef \max &\left\{
\lim_{k\rightarrow \pm \infty} \left| \frac{q_2(k)}{p_2(k)} \right|,
\max_{|k|>N,|k|\leq k' }\left| \frac{q_2(k)}{p_2(k)} \right| ,
%\right. \\&\left.
 \left| \frac{q_2(N+1)}{p_2(N+1)} \right|, \left| \frac{q_2(-N-1)}{p_2(-N-1)} \right|
\right\}.\end{split}
\end{align}
The limit $\lim_{k\rightarrow \pm \infty} \left| \frac{q_2(k)}{p_2(k)} \right|$ is trivial to determine and is non-zero only if $q_2$ and $p_2$ have the same polynomial order. All other bounds only require a finite computation.

With this algorithm, we can then bound explicitly the norm of an eventually diagonal operator as defined in \eqref{e:P}, \eqref{e:p}.



%</tail>
